Provably stable learning control of linear dynamics with multiplicative noise

Control of linear dynamics with multiplicative noise naturally introduces robustness against dynamical uncertainty. Moreover, many physical systems are subject to multiplicative disturbances. In this work we show how these dynamics can be identified from state trajectories. The least-squares scheme enables exploitation of prior information and comes with practical data-driven confidence bounds and sample complexity guarantees. We complement this scheme with an associated control synthesis procedure for LQR which robustifies against distributional uncertainty, guaranteeing stability with high probability and converging to the true optimum at a rate inversely proportional with the sample count. Throughout we exploit the underlying multi-linear problem structure through tensor algebra and completely positive operators. The scheme is validated through numerical experiments.

==> assets/unfoldtucker/unfoldtucker.tex <==
\definecolor{top-color}{HTML}{99D5C9}
\definecolor{front-color}{HTML}{6C969D}  
\definecolor{right-color}{HTML}{645E9D} 

\tikzset{
    xy cuboid/.pic={
        \tikzset{%
            /cuboid/.cd,
            #1
        }
        
        \draw[pic actions] 
            (0, 0, 0)                           coordinate (\cubelabel-luf)
            -- ++(0.5*\cubescale*\cubex, 0, 0)  coordinate (\cubelabel-cuf)
            -- ++(0.5*\cubescale*\cubex, 0, 0)  coordinate (\cubelabel-ruf) 
            -- ++(0, -0.5*\cubescale*\cubey, 0) coordinate (\cubelabel-rcf)
            -- ++(0, -0.5*\cubescale*\cubey, 0) coordinate (\cubelabel-rdf)
            -- ++(-0.5*\cubescale*\cubex, 0, 0) coordinate (\cubelabel-cdf)
            -- ++(-0.5*\cubescale*\cubex, 0, 0) coordinate (\cubelabel-ldf)
            -- ++(0, 0.5*\cubescale*\cubey, 0)  coordinate (\cubelabel-lcf)
            -- cycle (\cubelabel-luf);

        \node[pic actions, fill=none, draw=none] (\cubelabel-ccf) at ($(\cubelabel-ruf) - (0.5*\cubescale*\cubex, 0.5*\cubescale*\cubey)$) {\tikzpictext};
    },
    xz cuboid/.pic={
        \tikzset{%
            /cuboid/.cd,
            #1
        }
        
        \draw[pic actions] 
            (1, 0, 0)                           coordinate (\cubelabel-ruf)
            -- ++(-0.5*\cubescale*\cubex, 0, 0) coordinate (\cubelabel-cuf)
            -- ++(-0.5*\cubescale*\cubex, 0, 0) coordinate (\cubelabel-luf)
            -- ++(0, 0, -0.5*\cubescale*\cubez) coordinate (\cubelabel-luc)
            -- ++(0, 0, -0.5*\cubescale*\cubez) coordinate (\cubelabel-lub)
            -- ++(0.5*\cubescale*\cubex, 0, 0)  coordinate (\cubelabel-cub)
            -- ++(0.5*\cubescale*\cubex, 0, 0)  coordinate (\cubelabel-rub)
            -- ++(0, 0, 0.5*\cubescale*\cubez)  coordinate (\cubelabel-ruc)
            -- cycle (\cubelabel-ruf);

        \node [sloped, xslant=0.5, pic actions, fill=none, draw=none] (\cubelabel-cuc) at ($(\cubelabel-ruf) - (0.5*\cubescale*\cubex, 0, 0.5*\cubescale*\cubez)$) {\tikzpictext};
    },
    yz cuboid/.pic={
        \tikzset{%
            /cuboid/.cd,
            #1
        }
        
        \draw[pic actions] 
            (1, 0, 0)                           coordinate (\cubelabel-ruf)
            -- ++(0, -0.5*\cubescale*\cubey, 0) coordinate (\cubelabel-rcf) 
            -- ++(0, -0.5*\cubescale*\cubey, 0) coordinate (\cubelabel-rdf) 
            -- ++(0, 0, -0.5*\cubescale*\cubez) coordinate (\cubelabel-rdc)
            -- ++(0, 0, -0.5*\cubescale*\cubez) coordinate (\cubelabel-rdb)
            -- ++(0, 0.5*\cubescale*\cubey, 0)  coordinate (\cubelabel-rcb)
            -- ++(0, 0.5*\cubescale*\cubey, 0)  coordinate (\cubelabel-rub)
            -- ++(0, 0, 0.5*\cubescale*\cubez)  coordinate (\cubelabel-ruc)
            -- cycle (\cubelabel-ruf);
            
        \node [sloped, yslant=0.5, pic actions, fill=none, draw=none] (\cubelabel-rcc) at ($(\cubelabel-ruf) - (0, 0.5*\cubescale*\cubey, 0.5*\cubescale*\cubez)$) {\tikzpictext};
    },
    /cuboid/.search also={/tikz},
    /cuboid/.cd,
    width/.store in=\cubex,
    height/.store in=\cubey,
    depth/.store in=\cubez,
    units/.store in=\cubeunits,
    scale/.store in=\cubescale,
    label/.store in=\cubelabel,
    width=1,
    height=1,
    depth=1,
    units=cm,
    scale=1,
    label=cube-node
}

\begin{tikzpicture}    
    \pgfmathsetmacro{\localscale}{0.5}
    \pgfmathsetmacro{\modex}{1}
    \pgfmathsetmacro{\modey}{1}
    \pgfmathsetmacro{\modez}{1}
    \pgfmathsetmacro{\offset}{4.5}
    \pgfmathsetmacro{\shift}{4.25}

    % tensor ...............................................................
    \foreach \x in {0,...,1} {
        \foreach \z in {0,...,1} {
            \pic [fill=top-color, scale=\localscale] at ($\localscale*(\x, 0, -\z)$) {xz cuboid={label=cube-\x-0-\z}};
        }
    }

    \foreach \y in {0,...,1} {
        \foreach \z in {0,...,1} {
            \pic [fill=right-color, scale=\localscale] at ($\localscale*(1, -\y, -\z)$) {yz cuboid={label=cube-1-\y-\z}};
        }
    }

    \foreach \x in {0,...,1} {
        \foreach \y in {0,...,1} {
            \pgfmathtruncatemacro{\label}{1+2*\x + \y}
            \pic [fill=front-color, "$\label$", scale=\localscale] at ($\localscale*(\x, -\y, 0)$) {xy cuboid={label=cube-\x-\y-0}};
        }
    }

    \node[anchor=south east] at (cube-0-0-1-lub) {$\ten{T}$};

    % modes ............................................................
    \foreach \x in {1,...,2} {
        \foreach \z in {1,...,\modez} {
            \pic [fill=top-color, scale=\localscale] at ($\localscale*(\x-1, 0, -\z+1)+\localscale*(0, -2, \modez+0.75)$) {xz cuboid={label=mode2-\x}};
        }
    }

    \node[anchor=north, sloped, xslant=0.5] at (mode2-1-ruf) {$X_{2}$};

    \foreach \x in {1,...,\modex} {
        \foreach \z in {1,...,2} {
            \pic [fill=right-color, scale=\localscale] at ($\localscale*(\x-1, 0, -\z+1)+\localscale*(2.5, -2, 0)$) {xz cuboid={label=mode3-\z}};
        }
    }

    \node[anchor=south, sloped, xslant=0.5] at (mode3-2-cub) {$X_{3}$};

    \foreach \x in {1,...,\modey} {
        \foreach \y in {1,...,2} {
            \pic [fill=front-color, scale=\localscale] at ($\localscale*(\x-1, -\y+1, 0)+\localscale*(-\modey-0.5, 0, 0)$) {xy cuboid={label=mode1-\y}};
        }
    }

    \node[anchor=south] at (mode1-1-cuf) {$X_{1}$};

    % flattened ...........................................................
    \coordinate (cur) at ($\localscale*(2, 0, 0) + \localscale*(\offset, 0, 0)$);

    \foreach \x in {1,...,\modey} {
        \foreach \y in {1,...,2} {
            \pic [fill=front-color, scale=\localscale] at ($(cur) + \localscale*(\x-1, -\y+1, 0)+\localscale*(-\modey-0.5, 0, 0)$) {xy cuboid={label=mode1-\y}};
        }
    }

    \node[anchor=south] at (mode1-1-cuf) {$X_{1}$};

    \foreach \s in {0,...,1} {
        \foreach \x in {0,...,1} {
            \foreach \z in {0,...,0} {
                \pic [fill=top-color, scale=\localscale] at ($(cur) + \localscale*(\shift*\s, 0, 0) + \localscale*(\x, 0, -\z)$) {xz cuboid={label={cube\s-\x-0-\z}}};
            }
        }

        \foreach \y in {0,...,1} {
            \foreach \z in {0,...,0} {
                \pic [fill=right-color, scale=\localscale] at ($(cur) + \localscale*(\shift*\s, 0, 0) + \localscale*(1, -\y, -\z)$) {yz cuboid={label={cube\s-1-\y-\z}}};
            }
        }

        \foreach \x in {0,...,1} {
            \foreach \y in {0,...,1} {
                \pic [fill=front-color, scale=\localscale] at ($(cur) + \localscale*(\shift*\s, 0, 0) + \localscale*(\x, -\y, 0)$) {xy cuboid={label={cube\s-\x-\y-0}}};
            }
        }

        \foreach \x in {1,...,2} {
            \foreach \z in {1,...,\modez} {
                \pic [fill=top-color, scale=\localscale] at ($(cur) + \localscale*(\shift*\s, 0, 0) + \localscale*(\x-1, 0, -\z+1)+\localscale*(0, -2, \modez+0.75)$) {xz cuboid={label=mode2-\s-\x}};
            }
        }

        \pic [fill=none, draw=none, scale=\localscale, "\Large$\cdot$"] at ($(cur) + \localscale*(\shift*\s, 0, 0) + \localscale*(1.5, 0, 0)+\localscale*(0, -2, 1.75)$) {xz cuboid={width=0.5}};
        \pic [fill=right-color, scale=\localscale] at ($(cur) + \localscale*(\shift*\s, 0, 0) + \localscale*(2.5, 0, 0)+\localscale*(0, -2, 1.75)$) {xz cuboid={label=mode3-\s}};
    }

    % add labels
    \foreach \x in {0,...,1} {
        \foreach \y in {0,...,1} {
            \pgfmathtruncatemacro{\label}{1+2*\x + \y}
            \pic [draw=none, fill=none, scale=\localscale, "$\label$"] at ($(cur) + \localscale*(\x, -\y, 0)$) {xy cuboid};
        }
    }

    \draw [decorate,decoration={brace,amplitude=5pt,mirror,raise=4pt},yshift=0pt]
        (mode2-0-1-luf) -- (mode3-1-ruf) node [midway, yshift=-0.6cm] {$X_{3} \otimes X_{2}$};
    
    \draw [decorate,decoration={brace,amplitude=5pt,raise=4pt},yshift=0pt]
        (cube0-0-0-0-lub) -- (cube1-1-0-0-rub) node [midway, yshift=0.6cm] {$\ten{T}_{(1)} = [[\ten{T}]_{::1}, [\ten{T}]_{::2}]$}; 
\end{tikzpicture}
\vspace{-1em}

==> content/identification/ambiguity.tex <==
We would like to derive a suitable ambiguity set to solve the distributionally robust LQR problem \cref{eq:drlqr}. To do so
we first formalize the concept of an ambiguity set.

We operate in a setting similar to that of \cite{Coppens2021}. Specifically consider a probability space $(\Omega, \F, \prob)$ and the problem
\begin{align} \label{eq:sopt}
    \min_{u \in \set{U}} \quad \E[\ell(u, w)],
\end{align}
with $u \in \Re^{n_u}$ some decision variable, $\ell \colon \Re^{n_u} \times \Re^{n_w} \to \eRe$ some loss function and $w \colon \Omega \to \W$ a vector
with $\W \subset \Re^{n_w}$ the (compact) support of $w$. 

Letting $\Pf(\W)$ denote the space of probability measures on the measurable space $(\W, \B)$ with $\B$ the Borel $\sigma$-algebra associated with $\W$,
the main difficulty in solving \eqref{eq:sopt} is the \emph{push-forward} measure $\meas_{\star} \in \Pf(\W)$, defined as $\meas_{\star}(O) - \prob[w^{-1}(O)]$ for all $O \in \B$. 
In practice $\meas_{\star}$ is often unknown, hence $\E[\ell(u, w)] = \E_{\meas_{\star}}[\ell(u, w)]$ cannot be evaluated. 

Instead DRO considers an ambiguity set $\amb \subseteq \Pf(\W)$, which contains $\meas_{\star}$ with high confidence. 
That is 
\begin{equation} \label{eq:amb_conf}
        \prob[\meas_\star \in \amb] \geq 1 - \delta.
\end{equation}

Usually this is guaranteed by imposing some structure on $\amb$ \cite[Def.~II.1]{Coppens2021}. Examples are moment-based ambiguity, which constrain 
the measures in terms of its moments, Wasserstein ambiguity \cite{Kuhn2019} which is centered 
on the empirical measure and bounds the Wasserstein distance and $\phi$-divergence \cite{Schuurmans2020} which bounds 
some divergence. The Wasserstein sets has the issue that the radius $\beta$ depends on unknown parameters of the distribution and 
the $\phi$-divergence sets often only support discrete distributions. The advantage of moment-based ambiguity as considered here and in \cite{Coppens2021} is \emph{(i)} it contains 
measures that are not only supported on the data; \emph{(ii)} a fully data-driven estimate of $\beta$ is available; and \emph{(iii)} problem complexity does not 
grow with the sample count. For more info see \cite{Rahimian2019}.

% Specifically, we define a
% data-driven ambiguity as follows \cite[Def.~II.1]{Coppens2021},
% \begin{definition} \label{def:dd-amb}
%     Consider a random variable $w \colon \Omega \to \W$ with push-forward measure $\meas_{\star}$ and i.i.d. samples $\{w_i\}_{i \in \N_{1:M}}$. 
%     Let $\theta \in \Theta$ denote a statistic depending on the data and let 
%     $\beta \in \Re^{n_\beta}$ be some radii 
%     Then a \emph{data-driven ambiguity} 
%     $\amb \colon \Re^{n_\beta} \times \Theta \rightrightarrows \Pf(\W)$
%     with confidence $\delta \in (0, 1)$ maps $(\theta, \beta)$ 
%     to a closed, convex set $\amb_{\beta}(\hat{\theta}) \subseteq \Pf(\W)$
%     such that
%     \begin{equation} \label{eq:amb_conf}
%             \prob[\meas_\star \in \amb_{\beta}(\hat{\theta})] \geq 1 - \delta.
%     \end{equation}
% \end{definition}
% We specifically consider the setting where $\W = \{w \in \Re^{n_w} \colon \nrm{w}_2 \leq r\}$
% for some radius $r \geq 0$ and where the statistic $\theta$ acts as an estimate of $\smoment$. 
% This is referred to as moment-based ambiguity. A common alternative is using the empirical distribution as $\theta$, leading to Wasserstein ambiguity \cite{Kuhn2019}
% and $\phi$-divergence \cite{Schuurmans2020}. The first setting has the issue that the radius $\beta$ depends on unknown parameters of the distribution and 
% the second setting only supports discrete distributions. The advantage of the ambiguity considered here and in \cite{Coppens2021} is \emph{(i)} it contains 
% measures that are not only supported on the data; \emph{(ii)} a fully data-driven estimate of $\beta$ is available; and \emph{(iii)} problem complexity does not 
% grow with the sample count. A survey of ambiguity sets is given in \cite{Rahimian2019}.

For a concrete example, a direct application of a matrix Hoeffding bound (cf. \cref{lem:mathfd}) gives the following result when samples 
from the disturbance are available:
\begin{lemma} \label{lem:dd-moment}
    Let $\W = \left\{ w \in \Re^{n_w} \colon \nrm*{w}_2 \leq r_w \right\}$. 
    Assume we have a set of i.i.d. samples $\{w_i\}_{i\in\N_{1:M}}$ of a random vector $w$ and let
    $\smomenth \dfn \ssum_{i=1}^{\nsample} w_i \trans{w_i}/\nsample$.    
    Then
    \begin{equation*}
            \left\{ \meas \in \Pf(\W) \colon \nrm{\smomenth - \E_{\meas}[{w} \trans{{w}}]}_2 \leq \beta_{\cmoment} \right\}
    \end{equation*}
    satisfies \eqref{eq:amb_conf} when $\beta_{\smoment} = r^2_w \sqrt{2\ln(2n_w/\delta)/\nsample}$.
\end{lemma}

Given an ambiguity set $\amb$ we can then solve the following dro. problem, which is a conservative approximation of \eqref{eq:sopt},
\begin{equation} \label{eq:dropt}
    \min_{u \in \set{U}} \, \max_{\meas \in \amb} \, \E_{\meas}[\ell(u, w)].
\end{equation}
These problems are related to risk measures by duality \cite{Coppens2021}.

% In our setting we avoid this framework by optimizing over $\smoment$ instead of $\meas$.\todo{Remove this part?}
% Specifically, 
% when the cost function is quadratic we have the following result.
% \begin{lemma}
%     Problem \eqref{eq:dropt} with $\ell(u, w) = \trans{\hm{w}} Q(u) \hm{w}$ and $Q(u) \colon \Re^{n_u} \to \sym{\nwh}$
%     is equivalent to
%     \begin{align*}
%         &\min_{u \in \set{U}} \, \max_{\smoment \in \ambs \cap \ambr} \, \tr(Q(u) \smoment), \quad \text{with } \smoment = \begin{bmatrix}
%             \cmoment & \mean \\ \trans{\mean} & 1
%         \end{bmatrix}.
%     \end{align*}
%     with $\ambs = \{\smoment \in \psd{\nwh} \colon \nrm{\cmoment - \cmomenth}_2 \leq \beta_{\cmoment}, \nrm{\mean - \meanh}_2 \leq \beta_{\mean}\}$
%     and $\ambr = \{\smoment \in \psd{\nwh} \colon \tr[\cmoment] \leq r^2\}$.
% \end{lemma}
% \begin{proof}
%     The result formally follows by applying duality twice. First duality over measures to get rid of the maximization over $\meas$
%     as in \cite[Ex.~II.5]{Coppens2021} and then using SDP duality to return to a maximization over matrices. We can interpret the 
%     set $\ambr$ as imposing $\meas \in \Pf(\W)$. Specifically the trace bound is caused by the restriction of the support to $\W$. 
% \end{proof}
% \begin{lemma}
%     Problem \eqref{eq:dropt} with $\ell(u, w) = \trans{\hm{w}} Q(u) \hm{w}$ and $Q(u) \colon \Re^{n_u} \to \sym{\nwh}$
%     is equivalent to,
%     \begin{align*}
%         &\min_{u \in \set{U}} \, \max_{\smoment \in \ambs \cup \ambr} \, \tr(Q(u) \smoment),\\
%     \end{align*}
%     with moment ambiguity $\ambs = \{\smoment \in \psd{\nwh} \colon \nrm{\smoment - \smomenth}_2 \leq \beta, \}$ and
%     $\ambr = \{\smoment \in \psd{\nwh} \colon \tr([\smoment]_{1:n_w, 1:n_w}) \leq r^2, \, [\smoment]_{\nwh, \nwh} = 1\}$.
% \end{lemma}
% \begin{proof}
%     The result formally follows by applying duality twice. First duality over measures to get rid of the maximization over $\meas$
%     as in \cite[Ex.~II.5]{Coppens2021} and then using SDP duality to return to a maximization over matrices. We can interpret the 
%     set $\ambr$ as imposing $\meas \in \Pf(\W)$. Specifically $[\smoment]_{\nwh, \nwh} = 1$ imposes that $\meas$ is a
%     probability measure, while the trace bound is caused by the restriction of the support to $\W$. 
% \end{proof}

The goal now is to generalize \cref{lem:dd-moment} 
to the setting where only state measurements are available. 

==> content/identification/lqr.tex <==
The goal of this section is twofold \emph{(i)} we argue how LQ control of CP dynamics is equivalent 
to \cref{eq:slqr}; and \emph{(ii)} we show how the optimal policy is determined by solving a SDP,
generalizing the result of \cite{Balakrishnan2003}.  

We start by stating the CP equivalent of \cref{eq:slqr}
\begin{equation} \label{eq:lqrcp}
    \begin{alignedat}{2}
        &\minimize_{Z_t} &\quad& \sum_{t=0}^\infty \tr[Z_t H] \\
                             &\stt && Z_t = \begin{bmatrix}
                                 X_t & V_t \\ \trans{V_t} & U_t
                             \end{bmatrix} \sgeq 0, \\&&&X_{t+1} = \op{E}(Z_t), \quad \forall t \in \N,
    \end{alignedat} \tag{$\mathcal{LQR}_{\mathrm{cp}}$}
\end{equation}
with $H \dfn \blkdiag(Q, R) \sgt 0$. The psd. constraint on $Z_t$ ensures that it acts 
like the second moment of a random vector. 

% It is well known that the optimal policy for \eqref{eq:slqr} is linear: $u_t = K_\star x_t$ 
% for some $K_\star \in \Re^{n_u \times n_x}$ \cite{Coppens2019,Morozan1983}. 
% Selecting $H = \blkdiag(Q, R)$ and, as before, letting $X_t = \E[x_t \trans{x_t}]$, $U_t = \E[u_t \trans{u_t}] = K_\star X_t \trans{K}_\star$ 
% and $V_t = \E[x_t \trans{u_t}] = X_t \trans{K}_\star$ and using \cref{eq:dynsm_} shows that \eqref{eq:lqrcp} lower bounds 
% the cost of \cref{eq:slqr}. In fact, we can prove the stronger res:
We show that \eqref{eq:slqr} is equivalent to \eqref{eq:lqrcp}
\begin{proposition} \label{thm:cpmulteq}
    Let $\mathrm{Val}(\cdot)$ denote the optimal value. Then 
    \begin{equation*}
        \mathrm{Val}\eqref{eq:slqr} = \mathrm{Val}\eqref{eq:lqrcp},
    \end{equation*}
    given \cref{asm:model}. Moreover sequence $(Z_t)_{t \in \N}$ is feasible for \eqref{eq:lqrcp} iff there is a feasible sequence
    in \eqref{eq:slqr} $u_t = K_t x_t + \delta_t$ s.t.
    $Z_t = \E[z_t \trans{z_t}]$ where $z_t = (x_t, u_t)$. 
    Here $K_t \in \Re^{n_x \times n_u}$
    and $\delta_t \in \Re^{n_u}$ is a random vector $\forall t \in \N$.
\end{proposition}
\begin{proof}
    Deferred to Appendix~\ref{app:lqr}.
\end{proof}

To find the exact solution of \eqref{eq:lqrcp}, similarly 
to usual LQR, we need to consider a Riccati equation:
\begin{equation} \label{eq:ric-def}
    \op{R}(P) \dfn Q + \adj{\op{F}}(P) - \trans{(\adj{\op{H}})}(P)(R + \adj{\op{G}}(P))^{-1}\adj{\op{H}}(P).
\end{equation}
where $\adj{\op{F}}(P) = \ten{A}_{(2)} (\smoment \kron P) \trans{\ten{A}_{(2)}}$, 
$\adj{\op{G}}(P) = \ten{B}_{(2)} (\smoment \kron P) \trans{\ten{B}_{(2)}}$ and 
$\adj{\op{H}}(P) = \ten{B}_{(2)}(\smoment \otimes P) \trans{\ten{A}_{(2)}}$ with tensors $\ten{A}$ and $\ten{B}$ 
as in \cref{eq:dynten}. We use adjoint CP operators to be consistent with \cref{cor:cpadj}.

\begin{remark}
    The operators $\adj{\op{F}}$, $\adj{\op{H}}$ and $\adj{\op{G}}$ form
    the blocks of $\adj{\op{E}}$ when it is partitioned similarly to $Z_t$ (cf. \cref{lem:opadj}). 

    In the deterministic setting with $n_w = 1$ and $w_t = 1$ (so $\E[W] = 1$), we have $\adj{\op{F}}(P) = \trans{A}_1 P A_1$, $\adj{\op{H}}(P) = \trans{B}_1 P A_1$ and $\adj{G}(P) = \trans{B}_1 P B_1$.
    Hence we recover the classical Riccati operator as a special case. 
\end{remark}

We introduce the \emph{closed-loop operators} as
\begin{equation} \label{eq:clops}
    \Pi_K(X) \dfn [I; K] X [I, \trans{K}], \, \op{E}_K(X) \dfn \op{E}(\Pi_K(X)),
\end{equation}
The policy $Z_t = \Pi_K(X_t)$ is recovered when taking $u_t = Kx_t$ 
in the equivalent \eqref{eq:slqr} (cf. \cref{thm:cpmulteq}).

We can then state the following theorem.

\begin{theorem} \label{thm:cplqr}
    \shorten*{Let $\exists K\colon \rho(\op{E}_K) < 1$ and $H \dfn \blkdiag(Q, R) \sgt 0$.} Then 
    $Z_t = \Pi_{K_{\star}}(X_t)$ is \update*{an} optimal policy, 
        with $K_{\star} = -(R + \adj{\op{G}}(P_{\star}))^{-1} \adj{\op{H}}(P_{\star})$ and $P_{\star} \sgt 0$
        solves the Riccati equation $P_{\star} = \op{R}(P_\star)$. Moreover
    \begin{enumerate}
        \item \label{thm:cplqr:b} $\rho(\op{E}_{K_\star}) < 1$; 
        \item $\mathrm{Val}\eqref{eq:lqrcp} = \tr[P_{\star} X_0]$;
        % \item \label{thm:cplqr:d} $P_\star  \in \argmax \left\{\tr[P X_0] \colon \adj{\op{L}}(P) \sleq H, P \sgeq 0 \right\}$.\\
        %                                     The solution to this SDP is unique if $X_0 \sgt 0$. 
    \end{enumerate}
\end{theorem}
\begin{proof}
    \ilarxiv{See Appendix~\ref{app:lqr} for the full proof.}\ilpub{This result was shown for multiplicative noise in \cite{Coppens2019, Morozan1983} 
    and generalized to the CP setting by \cref{thm:cpmulteq}. Nonetheless, a full proof is included in the technical report \citear{}.}
\end{proof}

\begin{prepupdate}
    \begin{remark} \label{rem:stabilizability}
        Here $\exists K \colon \rho(\op{E}_K(\cdot)) < 1$ 
        is referred to as \emph{stabilizability}. Among other things 
        it implies the system being below the \emph{uncertainty threshold} \cite{Athans1977}.
    \end{remark}
\end{prepupdate}

\begin{arxiv}
    \begin{example}
        Let us consider a deterministic system with $n_w = 1$ and
        \begin{equation*}
            A_1 = \begin{bmatrix}
                1 & 0.1 \\ 
                0 & 1
            \end{bmatrix}, \, B_1 = \begin{bmatrix}
                0 \\ 0.1
            \end{bmatrix}.
        \end{equation*}
        This will help us understand how \cref{eq:lqrcp} generalizes the usual notions of LQR. We pick $H = \diag(1, 1, 0.1)$. Then 
        the solution described by \cref{thm:cplqr} is approximately:
        \begin{equation*}
            K = [-1.75, -2.64].
        \end{equation*}
        One can easily verify that this is the usual LQR solution in the deterministic setting. Let's spend some time noting what happens when 
        we set $X_0 = x_0 \trans{x_0}$. In that case, for some $u_0$, let $Z_0 = (x_0, u_0) \trans{(x_0, u_0)}$. Then (similarly to \cref{ex:smdyn}):
        \begin{align*}
            \op{E}(Z_0) &= A_1 x_0 \trans{x_0} \trans{A}_1 + A_1 x_0 \trans{u_0} \trans{B_1} \\ &\qquad + B_1 u_0 \trans{x_0} \trans{A}_1 + B_1 u_0 \trans{u_0} \trans{B_1}.
        \end{align*}
        It is not difficult to verify that this equals $x_1 \trans{x_1}$ for $x_1 = A_1 x_0 + B_1 u_0$. We could repeat this for each time step 
        noting that $X_t = x_t \trans{x_t}$ and $Z_t = (x_t, u_t) \trans{(x_t, u_t)}$ in \cref{eq:lqrcp}. Trivially we have $Z_t \sgeq 0$,
        so the trajectory is feasible. Moreover the cost becomes $\tr[Z_t H] = \trans{x_t} I x_t + 0.1 \trans{u_t} I u_t$. So we can see 
        that the classical LQR controller is at least a feasible solution to \cref{eq:lqrcp} where we then have 
        \begin{align*}
            Z_t = \Pi_K(X_t) &= \begin{bmatrix}
                x_t \trans{x_t} & x_t \trans{x}_t \trans{K} \\ K x_t \trans{x_t} & K x_t \trans{x}_t \trans{K}
            \end{bmatrix} \\ &= (x_t, Kx_t) \trans{(x_t, Kx_t)}.
        \end{align*}
        Note that we have shown in \cref{thm:cplqr} that such policies are in fact optimal. In terms of classical LQR this 
        implies that, a random policy $u_t = Kx_t + \delta_t$ for some random $\delta_t$ will not improve performance. 
    \end{example}
\end{arxiv}

% We are specifically interested in the case $N \to \infty$. 
% \begin{theorem} \label{thm:_cplqr}
%     Consider \eqref{eq:lqr-finite}. Assume $\exists K\colon \rho(\op{E}_K) < 1$ and $H \sgt 0$. Then
%     the optimal policy is $Z_t = \Pi_{K_{\star}}(X_t)$, 
%         with $K_{\star} = -(R + \adj{\op{G}}(P_{\star}))^{-1} \adj{\op{H}}(P_{\star})$ and $P_{\star} \sgt 0$
%         solves the Riccati equation $P_{\star} = \op{R}(P_\star)$. Moreover
%     \begin{enumerate}
%         \item \label{thm:_cplqr:b} $\rho(\op{E}_{K_{\star}}) < 1$; 
%         \item $\op{J}^\star(X_0) = \tr[P_{\star} X_0]$;
%         \item \label{thm:_cplqr:d} $P_\star  \in \argmax \left\{\tr[P X_0] \colon \adj{\op{L}}(P) \sleq H, P \sgeq 0 \right\}$.\\
%                                             The solution to this SDP is unique if $X_0 \sgt 0$. 
%     \end{enumerate}
%     Here $\op{L}(Z)$ is as defined in \cref{eq:lyapdef}. The operators $\adj{\op{F}}, \adj{\op{G}}$ and $\adj{\op{H}}$ 
%     are as in \cref{eq:ope-partition}. 
% \end{theorem}
% \begin{proof}
%     See the proof in Appendix~\ref{app:lqr}.
% \end{proof}
% \begin{remark}
%     The uniqueness result \cref{thm:cplqr:d} indicates the need for regularization. That is, instead of taking $X_0 = x_0 \trans{x_0}$
%     for a deterministic initial state we will consider $X_0 = x_0 \trans{x_0} + \lambda I$ for some small $\lambda > 0$. 
% \end{remark}
% \begin{remark}
%     The constraint of the SDP in \cref{thm:cplqr:d} is
%     \begin{equation*}
%         \begin{bmatrix}
%             Q - P + \ten{A}_{(2)} (\smoment \kron I) \trans{\ten{A}_{(2)}} & \ten{A}_{(2)} (\smoment \kron I) \trans{\ten{B}_{(2)}} \\ 
%             \ten{B}_{(2)} (\smoment \kron I) \trans{\ten{A}_{(2)}} & R + \ten{B}_{(2)} (\smoment \kron I) \trans{\ten{B}_{(2)}}
%         \end{bmatrix} \sgeq 0.
%     \end{equation*}
%     The result is therefore equivalent to that of \cite[Prop.~3]{Coppens2021} and is direct generalization 
%     of the continuous time reformulation of \cite[\S{}V]{Balakrishnan2003} to discrete time when $n_w = 0$. 
% \end{remark}


% One issue with the SDP considered in \cref{thm:cplqr} is that the feasible solutions $P$ will not necessarily lead to
% stabilizing controllers. Therefore, when considering distributionally robust synthesis we will consider the following problem:
% \begin{equation} \label{eq:stab-sdp}
%     \minimize_{(P, K)} \, \{\tr[P X_0] \colon \adj{\op{L}}(K; P) \sgeq \adj{\Pi}(K; H), P \sgeq 0 \},
% \end{equation}
% the constraint of which is a Lyapunov constraint, thereby imposing stability through \cref{prop:lyapcp}. 
% We can show:
% \begin{proposition} \label{prop:stablqr}
%     The problem \eqref{eq:stab-sdp} satisfies:
%     \begin{enumerate}
%         \item \label{prop:stablqr:a} $\rho(\op{E}_K) < 1$ for any feasible $K$;
%         \item $(P_\star, K_{\star})$ is optimal and uniquely so if $X_0 \sgt 0$.
%     \end{enumerate}
% \end{proposition}
% \begin{proof}
%     See the proof in Appendix~\ref{app:lqr}.    
% \end{proof}

Even though we directly tackled second moment dynamics in \cref{thm:cplqr}, 
the optimal policy $Z_t = \Pi_{K_{\star}}(X_t)$ 
is realizable for multiplicative noise dynamics using 
$u_t = K_{\star} x_t$. So this controller is also optimal 
for \eqref{eq:slqr} as is well known (cf. \cite[Prop.~3]{Coppens2019})
and achieves the equality in \cref{thm:cpmulteq}. 

Thus we can conclude that LQR of CP dynamics
is (i) identical to LQR of multiplicative noise dynamics; (ii) 
a natural generalization of classical LQR; and (iii) a relaxation for LQR of 
switching systems in the sense of \cref{thm:stab-eq}. 

The final question is how to find a $P_\star$ satisfying \eqref{eq:ric-def}. Numerical solution 
of such equations is considered in detail in \cite{Damm2003}. We consider a reformulation
as a SDP, akin to \cite{Balakrishnan2003}. 

\begin{theorem} \label{thm:ric-sdp-primal}
    Let $P_\star$ solve the Riccati equation \eqref{eq:ric-def}. Then $P_\star$
    is a maximizer of
    \begin{equation*}
        \begin{alignedat}{2} 
            &\maximize_{P \sgeq 0} &\quad& \tr[P X_0] \\
            &\stt && \begin{bmatrix}
                P - \adj{\op{F}}(P) & -\trans{(\adj{\op{H}})}(P) \\
                -\adj{\op{H}}(P) & -\adj{\op{G}}(P)
            \end{bmatrix} \sleq \begin{bmatrix}
                Q \\ & R
            \end{bmatrix},
        \end{alignedat}
    \end{equation*}
    with $\adj{\op{F}}$, $\adj{\op{H}}$ and $\adj{\op{G}}$ as defined below \eqref{eq:ric-def}. 
    Moreover, when $X_0 \sgt 0$, then $P_\star$ is the unique solution.
\end{theorem}
\begin{proof}
    The proof is analogous to the one in \cite{Balakrishnan2003} and \cite[Prop.~3]{Coppens2019}. \ilarxiv{The full proof is Deferred to Appendix~\ref{app:lqr}.}\ilpub{A full proof in the CP case is Deferred to \citear{}.}
\end{proof}

\update*{When the dynamics are not stabilizable, the SDP in \cref{thm:ric-sdp-primal}
will not have a positive definite solution for $X_0 \sgt 0$.}

==> content/identification/old/informativity.tex <==
We describe the error model and that, the estimators provide an unbiased estimate of the second moment dynamics. 

The error of both estimators is given as:
\begin{align*}
    \mean - \meanh &= (I - \pinv{\opm{Z}_{\mean}} \opm{Z}_{\mean}) \mean + \dots \text{ and} \\
    \svec(\cmoment - \cmomenth) &= (I - \pinv{\opm{Z}_{\cmoment}} \opm{Z}_{\cmoment}) \svec(\cmoment) + \dots
\end{align*}
We omit the zero-mean terms for now, which will be investigated in the next sections. We now investigate the other term.

We will make the following assumption:
\begin{assumption} \label{asm:nondeg}
     Assume $\rk(\ten{M}_{(3)}) = n_w$. 
\end{assumption}

% We can prove an auxiliary result for $\ten{M} \kron \ten{M}$.\todoright{this is useless\dots}
% \begin{lemma} \label{lem:nondeg}
%     Given \cref{asm:nondeg}, then $\rk((\ten{M} \kron \ten{M})_{(3)}) = n_w^2$. 
% \end{lemma}
% \begin{proof}
%     Assume there is some $W \in \Re^{n_w \times n_w}$ s.t. $W \neq 0$ and 
%     \begin{equation} \label{eq:kernel1}
%         \trans{\vec}{(W)}(\ten{M} \kron \ten{M})_{(3)} = 0,
%     \end{equation}
%     which holds iff. $\trans{\vec}{(W)}(\ten{M} \kron \ten{M})_{(3)} (\vec(Z) \kron \vec(X)) = \tucker{\ten{M} \kron \ten{M}; \vec(X), \vec(Z), \vec(W)}= 0$,
%     $\forall X \in \Re^{n_x \times n_x}$ and $Z \in \Re^{n_z \times n_z}$.
%     So by \cref{prop:cpunfold}, \eqref{eq:kernel1} holds iff.
%     \begin{align}
%         &&\tr[W \ten{M}_{(3)} (Z \kron X) \trans{\ten{M}_{(3)}}] &= 0, \, \forall Z, X \nonumber \\
%         \Leftrightarrow&& \tr[\trans{\ten{M}_{(3)}} W \ten{M}_{(3)} (Z \kron X)] &= 0, \, \forall Z, X \nonumber \\
%         \Leftrightarrow&& \trans{v} \trans{\ten{M}_{(3)}} W \ten{M}_{(3)} u &=0, \, \forall v, u \in \Re^{n_z n_x} \label{eq:kernel2}
%     \end{align}
%     Here the final equivalence follows by noting that any $v = v_z \kron v_x$ for some $v_x \in \Re^{n_x}$ and $v_z \in \Re^{n_z}$ 
%     and similarly let $u = u_z \kron u_x$. Then letting $Z = u_z \trans{v_z}$ and $X = u_x \trans{v_x}$. Then $Z \kron X = u \trans{v}$. 
%     Eq. \eqref{eq:kernel2} then follows by cyclicity of the trace. 

%     From \cref{asm:nondeg} $\ten{M}_{(3)}$ is full rank, so \eqref{eq:kernel2} holds iff $W = 0$, which by contradiction confirms the required result. 
% \end{proof}

Note that, by \cref{lem:zopeq} and letting $\ten{W} \dfn \ten{M} \skron \ten{M}$:
\begin{align}
    \opm{Z}_\mean &= (\trans{[z_1, z_2, \dots, z_N]} \kron I_{n_x}) \trans{\ten{M}_{(3)}} \label{eq:opzmean-stacked}\\
    \opm{Z}_\cmoment &= (\trans{[z_1 \skron z_1, \dots, z_N \skron z_N]} \kron I_{\sd{n_x}}) \trans{\ten{W}}_{(3)}. \label{eq:opzcmoment-stacked}
\end{align}
We know by \cref{asm:data} and \cref{lem:rank-condition} that $[z_1, z_2, \dots, z_N]$ is full rank, for sufficiently large $N$ 
and by \cref{asm:nondeg}, $\ten{M}_{(3)}$ is full rank. Therefore $\opm{Z}_{\mean}$ is left invertible and $I - \pinv{\opm{Z}_{\mean}}\opm{Z}_{\mean} = 0$:

\begin{corollary} \label{cor:nondeg}
    Given $N \geq n_z$, and following \cref{asm:data,asm:nondeg}, then $\opm{Z}_\mean$ is a.s. left invertible.
    Therefore $\E[\meanh - \mean] = 0$ a.s.\footnote{%
        In this section, we will often state a.s. results in terms of the expectation of estimates. 
        The a.s. is taken over the data $(z_i, y_i)_{i=1}^N$ and the expectation 
        taken over the (unobservable) noise $(w_i)_{i=1}^N$. %
    }
\end{corollary}

Given \cref{cor:nondeg} one might hope that $\hat{W}$ is also unbiased. In fact, one can show that, given \cref{asm:nondeg},
$\rk[(\ten{M} \kron \ten{M})_{(3)}] = n_w^2$. However, the same is not true for $\ten{M} \skron \ten{M}$.
%However, letting $n_x = 3$, $n_z = 6$ and $n_w = 6$ implies that $(\ten{M} \skron \ten{M})_{(3)} \in \Re^{21 \times 3 \cdot 6}$, which means it cannot be of rank $\sd{n_w} = 21$. 
% So even though $(\ten{M} \kron \ten{M})_{(3)}$ is full rank under \cref{asm:nondeg}, the same is not always true for $(\ten{M} \skron \ten{M})_{(3)}$. 
Simply replacing $\ten{M} \skron \ten{M}$ by $\ten{M} \kron \ten{M}$ is also not an option. Then we need to 
use $[z_1 \kron z_1, \dots, z_N \kron z_N]$ in $\opm{Z}_{\cmoment}$, which does not become full rank for sufficiently large $N$. 

Hence, for several bases of interest, including model-free ones (cf. \cref{rem:basis}), $\opm{Z}_{\cmoment}$ will never become left invertible. 
A similar phenomena was already observed in \cite{Xing2021}. This, beyond an unfortunate complication in the analysis, 
causes no issues when considering LQR. Specifically, we argue that, even though the estimate of $\cmoment$ 
might be biased, the estimate of the second moment dynamics $\op{E}$ is not. 

We begin with an auxiliary lemma:
\begin{lemma} \label{lem:kernel-mode3}
    Given \cref{asm:data} and $N \geq \sd{n_w}$. Then
    \begin{equation} \label{eq:kernel-mode3}
        \tucker{\ten{W}; \svec(\E[\hat{W} - W])} = 0.
    \end{equation}
\end{lemma}
\begin{proof}
    Letting $\Delta \cmoment \dfn \E[\hat{W} - W]$, from the error model in the beginning of this section
    \begin{align} \label{eq:cmoment-err}
        \svec(\Delta \cmoment) = (I - \pinv{\opm{Z}_{\cmoment}} \opm{Z}_{\cmoment}) \svec(\cmoment).
    \end{align}
    Using \eqref{eq:opzcmoment-stacked}, \cref{asm:data} and \cref{cor:rank-kron-condition} we know that 
    $(I - \pinv{\opm{Z}_{\cmoment}} \opm{Z}_{\cmoment}) = (I - \pinv{(\trans{\ten{W}_{(3)}})} \trans{\ten{W}_{(3)}})$. 
    Hence $\ten{W}_{(3)} \svec(\Delta \cmoment) = 0$, which implies \eqref{eq:kernel-mode3} by \cref{prop:kronunfold}. 
\end{proof}

We can now formalize unbiasedness of our estimate of $\op{E}$:
\begin{proposition} \label{prop:unbiased}
    Given \cref{asm:data,asm:nondeg}, $N \geq \sd{n_w}$ and let $\hat{\op{E}}$ be the dynamics \eqref{eq:e-op-def} using $\cmomenth$ and $\mean$. 
    Then $\E[\hat{\op{E}} - \op{E}] = 0$ a.s.
\end{proposition}
\begin{proof}
    Henceforth, let $\Delta W \dfn \E[\cmomenth - \cmoment]$.
    Note that $\hat{\op{E}}$ is linear in $\meanh$. Hence, by \cref{cor:nondeg}, $\E[\meanh] = \meanh$. 
    So, writing out \cref{eq:e-op-def} using this fact, we only require:
    \begin{align*}
       && \tr[P \ten{M}_{(1)} (\E[\cmomenth - \cmoment] \kron Z) \trans{\ten{M}_{(1)}}] &= 0 \\
       \Leftrightarrow && \tucker{\ten{W}; \svec(P), \svec(Z), \svec(\Delta \cmoment)} &= 0,
    \end{align*}
    for all $P \in \sym{n_x}$ and $Z \in \sym{n_z}$, where the equivalence follows by \cref{prop:cpunfold}.
    Using \cref{lem:kernel-mode3}, we can see that this holds a.s. over the data.
\end{proof}

To avoid unnecessary complexity, we will instead assume:
\begin{assumption} \label{asm:nondeg-cmoment}
    Assume $\svec(W) \in \img(\ten{W}_{(3)})$,
\end{assumption}
with the direct consequence (by the earlier analysis) that:
\begin{corollary} \label{cor:nondeg-cmoment}
    Given $N \geq \sd{n_z}$, and following \cref{asm:data,asm:nondeg-cmoment}.
    Then $\E[W - \hat{W}] = 0$ a.s. 
\end{corollary}

Keep in mind that \cref{asm:nondeg-cmoment} is without loss of generality in the sense of \cref{prop:unbiased}.
Specifically, if \cref{asm:nondeg-cmoment} does not hold, then $\hat{W}$ will be the closest estimate (in $\nrm{\cdot}_F$) 
of $W$ in $\img(\ten{W}_{(3)})$, such that $\hat{\op{E}}$ remains unbiased. 

Armed with \cref{cor:nondeg} and \cref{cor:nondeg-cmoment} we can now tackle the zero-mean part
and the sample complexity. 

% \begin{lemma} \label{lem:rank-convergence}
%     If $N \geq n_z$, then $I - \pinv{\opm{Z}_{\mean}} \opm{Z}_{\mean}$ projects onto the kernel of $\trans{\ten{M}_{(1)}}$ a.s.
%     Similarly if $N \geq n_z^2$, then $I - \pinv{\opm{Z}_{\cmoment}} \opm{Z}_{\cmoment}$
%     projects onto the kernel of $\trans{(\ten{M} \skron \ten{M})_{(1)}}$ a.s.
% \end{lemma}
% \begin{proof}
%     Let $Z_N \dfn [z_1; \dots; z_N]$ and $Z_{\kron, N} \dfn [z_1 \skron z_1; \dots; z_N \skron z_N]$. From \cref{lem:zopeq}, \cref{prop:kronunfold} 
%     and noting that $[(\trans{a} \otimes I); (\trans{b} \otimes I)] = \trans{[a; b]} \otimes I$ for any $a,b \in \Re^d$ gives, for $\ten{W} \dfn \ten{M} \skron \ten{M}$. 
%     \begin{equation*}
%         \opm{Z}_{\mean} = (\trans{Z_N} \otimes I) \trans{\ten{M}_{(1)}}, \quad \opm{Z}_{\cmoment} = (\trans{Z_{\kron, N}} \otimes I) \trans{\ten{W}_{(1)}},
%     \end{equation*}
        
%     By \cref{lem:rank-condition} and \cref{cor:rank-kron-condition} we have $\rk{(Z_N)} = n_z$ a.s. for $N \geq n_z$
%     and $\rk{(Z_{\otimes, N})} = n_z^2$ for $N \geq n_z^2$. This, by \cite[Thm.~4.2.15]{Horn1991}, implies that $\trans{Z_N} \otimes I$
%     and $\trans{Z_{\kron, N}} \otimes I$ are full rank. So they are also left invertible. Hence
%     \begin{equation*}
%         \pinv{\opm{Z}_{\mean}} \opm{Z}_{\mean} = \pinv{(\trans{\ten{M}_{(1)}})} (\trans{\ten{M}_{(1)}}), \quad
%         \pinv{\opm{Z}_{\cmoment}} \opm{Z}_{\cmoment} = \pinv{(\trans{\ten{W}_{(1)}})} (\trans{\ten{W}_{(1)}}).
%     \end{equation*}
%     The result follows from properties of the pseudo-inverse.
% \end{proof}

% Therefore, to avoid bias, we make an additional assumption:
% \begin{assumption}\label{asm:pe}
%     Assume $\mean \in \img(\ten{M}_{(1)})$ and $\cmoment \in \img(\ten{W}_{(1)})$. 
% \end{assumption}

% We however note that, this assumption in some sense is made without loss of generality. We make this explicit:
% \begin{proposition} \label{prop:asm-eq}
%     Let $\smoments = \smoment + \smoment'$, with partitioned terms
%     \begin{equation*}
%         \smoment \dfn \begin{bmatrix}
%             {\cmoment} & {\mean} \\ \trans{\mean} & 1
%         \end{bmatrix}, \quad \smoment' \dfn \begin{bmatrix}
%             {\cmoment}' & {\mean}' \\ \trans{(\mean')} & 0
%         \end{bmatrix}
%     \end{equation*}
%     for $\mean \in \img(\ten{M}_{(1)})$, $\svec(\cmoment) \in \img(\ten{W}_{(1)})$, $\mean' \in \ker(\trans{\ten{M}_{(1)}})$ and $\svec(\cmoment') \in \ker(\trans{\ten{W}_{(1)}})$.

%     Then $\op{E}(\smoments; Z) = \op{E}(\smoment; Z)$, $\forall Z \in \psd{n_z}$. 
% \end{proposition}
% \begin{proof}
%     For all $P \sgeq 0$ and random $z$ with $\E[z \trans{z}] = Z$,
%     \begin{align*}
%         &\tr[P(\op{E}(\smoments; Z) - \op{E}(\smoment; Z))] \\
%             &\qquad= \tr[\E[P\hm{\ten{M}}_{(3)} (z \otimes I) \smoment' (\trans{z} \otimes I) \trans{\hm{\ten{M}}_{(3)}}]] \\
%             &\qquad= \tr[\E[P(\trans{z} \otimes I) \trans{\hm{\ten{M}}_{(1)}} \smoment' \hm{\ten{M}}_{(1)} (z \otimes I)]] \\
%             &\qquad= \tr[ (Z \otimes P) \trans{\hm{\ten{M}}_{(1)}} \smoment' \hm{\ten{M}}_{(1)}],
%     \end{align*}
%     where the second equality follows by \eqref{eq:dyn1}.
    
%     We first show $\trans{\hm{\ten{M}}_{(1)}} \smoment' \hm{\ten{M}}_{(1)} = \trans{\ten{M}_{(1)}} \cmoment' \ten{M}_{(1)}$. 
%     Note $\trans{\hm{\ten{M}}_{(1)}} = [\trans{\ten{M}}_{(1)}, \bm{m}]$,
%     with $\bm{m} \dfn \vec([\hm{\ten{M}}]_{\nwh::})$.
%     by definition of the $n$-mode flattening \cite{Kolda2009}. So $\trans{\hm{\ten{M}}_{(1)}} \smoment' \hm{\ten{M}}_{(1)}$ equals
%     \begin{align*}
%         \trans{\ten{M}_{(1)}} \cmoment' \ten{M}_{(1)} + (\bm{m} \trans{(\mean')}) \ten{M}_{(1)} 
%         + \trans{\ten{M}_{(1)}} (\mean' \trans{\bm{m}}).
%     \end{align*}
%     The last terms two are zero, by $\mean' \in  \ker(\trans{\ten{M}_{(1)}})$. 
    
%     So it is sufficient to show $\tr[\ten{M}_{(1)} (Z \otimes P)  \trans{\ten{M}_{(1)}} \cmoment'] = 0$. 
%     By \cref{lem:zopexp:a}, the l.h.s. equals \[\E[\tr[\trans{\op{Z}}(z) P {\op{Z}}(z) \cmoment']] = \E[\tr[P {\op{Z}}(z) \cmoment' \trans{\op{Z}}(z)]].\]
%     Applying \eqref{eq:skronfund}, gives $\op{Z}(z) \cmoment' \trans{\op{Z}}(z)  = 0$ iff.
%     \begin{align*}
%         \op{Z}_{\otimes}(z) \svec(\cmoment') = (\trans{(z \otimes z)} \otimes I) \trans{\ten{W}}_{(1)} \svec(\cmoment') = 0,
%     \end{align*}
%     where we used \cref{lem:zopeq:b}. The final equality holds by  $\svec(\cmoment') \in \ker(\trans{\ten{W}_{(1)}})$, completing the proof.
% \end{proof}

% Intuitively, \cref{prop:asm-eq} implies that \cref{asm:pe} will have no effect on the second moment dynamics. Since the LQR controller
% only depends on $\op{E}$, we can thus claim that \cref{asm:pe} is without loss of generality.

% For the estimators to converge to the true values we need
% \begin{equation*}
%     \pinv{\opm{Z}_{\mean}} \opm{Z}_{\mean} \mean = \mean \quad \text{and} \quad \pinv{\opm{Z}}_{\cmoment} \opm{Z}_{\cmoment} \svec{\cmoment} = \svec{\cmoment}.
% \end{equation*}
% In this case the error is entirely controlled by a sum of i.i.d. bounded random vectors (matrices), which we bound using a Hoeffding bound in the next section. 
% The above conditions imply that $\mean$ and $\svec(\cmoment)$ lie in the row spaces of $\opm{Z}_{\mean}$ 
% and $\opm{Z}_{\cmoment}$. Therefore we operate on the following assumption:
% \begin{assumption} \label{asm:pe}
%     We assume, for all $\nsample \geq \nsample_0 \dfn \sd{n_z}$, that
%     $\mean \in \row(\opm{Z}_{\mean})$ and $\cmoment \in \row(\opm{Z}_{\cmoment})$. 
% \end{assumption} 

% \begin{remark} \label{rem:asm-pe}
%     This assumption does not reduce the practicality of our method,
%     due to \cref{asm:data}. We do so by illustrating that the kernel of $\opm{Z}_{\mean}$
%     and $\opm{Z}_{\cmoment}$ do not affect the second moment dynamics when sufficient data is gathered
%     in Appendix~\ref{app:identification}. 

%     Since the LQR only depends on the first and second moments of the states, it is therefore sufficient to
%     consider a $\mean$ and $\cmoment$ satisfying \cref{asm:pe}. 
% \end{remark}\trans{z}

==> content/identification/old/mean-bounds.tex <==
In this section we derive a data-driven ambiguity set as in \cref{def:dd-amb} centered on $\meanh$ derived above. 
We also derive radii depending on $\nsample$.

\paragraph{Data-driven bound} In the discussion from the previous section, we omitted the zero-mean terms. These are given as:
\begin{equation*}
    \mean - \meanh = \ldots +  \ssum_{i=1}^{\nsample} H_i \epsilon_i,
\end{equation*}
with $H_i \dfn \pinv{(\ssum_{j=1}^{\nsample} \trans{\op{Z}}(z_j) \op{Z}(z_j))} \trans{\op{Z}}(z_i) \op{Z}(z_i)$.
So, under \cref{asm:nondeg}, the error is given by a sum of norm-bounded zero-mean independent random vectors. 
\begin{proposition} \label{lem:mean-dd}
    We follow \cref{def:ls-est} and \cref{asm:data}--\ref{asm:nondeg} with $N \geq n_z$. 
    Let $\meanh = \pinv{\opm{Z}}_{\mean} Y_{\mean}$ and $\zeta^2_{\mean} \dfn \ssum_{i=1}^N \nrm{V^{1/2} H_i}_2^2$. Then,
    \begin{equation*}
        \prob[\trans{(\mean - \meanh)} V (\mean - \meanh) \leq \beta_{\mean}^2] \geq 1-\delta,
    \end{equation*}
    with $\beta_{\mean} = r \zeta_{\mean}  (2 + \sqrt{2 \ln(1/\delta)})$.
\end{proposition}
\begin{proof}
    By \cref{cor:nondeg}, a.s. over the data,
    \begin{equation*}
        V^{1/2}(\mean - \meanh) = \ssum_{i=1}^{\nsample} V^{1/2} H_i \epsilon_i = \ssum_{i=1}^{\nsample} v_i,
    \end{equation*}
    with $\nrm{v}_i \leq \nrm{V^{1/2} H_i}_2 r$ a (by \cref{asm:data}) independence 
    sequence of random vectors for $i=1, \dots, \nsample$. Applying \cref{lem:vechfd} with $[\gamma]_i = \nrm{V^{1/2} H_i}_2 r$, 
    and squaring both sides gives the required result.   
\end{proof}

\begin{remark}
    We introduce the normalization matrix $V$ to allow reshaping of the ambiguity. 
    A common choice is $V = \ssum_{j=1}^{\nsample} \trans{\op{Z}}(z_j) \op{Z}(z_j)/N$ (cf. \cite{Abbasi-Yadkori2011e}).
\end{remark}

\paragraph{Sample complexity} 
Due to independence one may expect that all matrices $\trans{\op{Z}}(z_i) \op{Z}(z_i)$ behave similarly. Hence one can expect that $\nrm{H_i}$ 
will decrease with $1/N$. So $\zeta_{\mean}$ would decrease with $1/\sqrt{N}$. We formalize this in a simplified setting.
\begin{lemma} \label{lem:mean-sample-complexity}
    We follow \cref{def:ls-est} and \cref{asm:data}--\ref{asm:nondeg} with $N \geq n_z$
    and assume additionally that $\nrm{z_i}_2 \leq r_z$ a.s. for all $i \in \N_{1:N}$. Then, if  $N \geq (\nrm{\ten{M}}_2^2 \tau_{\mean}/ \gamma_{\mean})^2$,
    \begin{equation*}
        \prob\left[\zeta_{\mean} \leq \frac{\nrm{\ten{M}}_2^2}{\sqrt{N} \gamma_{\mean} - \nrm{\ten{M}}_2^2 \tau_{\mean}}\right] \leq \delta,
    \end{equation*}    
    with $\tau_{\mean} \dfn \sqrt{2\ln(2 n_w/\delta)}$
    and \[\gamma_{\mean} \dfn \lambda_{n_w}\left[\ten{M}_{(1)} \left({\E[z \trans{z}]}/{r_z^2} \otimes I\right) \trans{\ten{M}}_{(1)}\right].\]
\end{lemma}
\begin{proof}
    For all $i \in \N_{1:\nsample}$, consider the i.i.d. random matrices $Y_i = \trans{\op{Z}}(z_i) \op{Z}(z_i)$, $\Delta_i = Y_i - \E[Y_i]$ 
    and $Y \dfn \ssum_{i=1}^{\nsample} Y_i$. 
    We have $\E[Y_i] = \E[\trans{\op{Z}} \op{Z}]$
    and $\nrm{Y_i}_2 \leq r_z \nrm{\op{Z}}_2^2$ . Since $-r_z \nrm{\op{Z}}_2^2 I \sleq -\E[Y_i] \sleq \Delta_i \sleq Y_i \sleq r_z^2 \nrm{\op{Z}}_2^2 I$,
    we have $\nrm{\Delta_i}_2 \leq r_z^2 \nrm{\op{Z}}_2^2 \leq r_z^2 \nrm{\ten{M}}_2^2$ (cf. \cref{lem:zopnorm}). A direct application of \cref{lem:mathfd} gives
    \begin{equation*}
        \prob[\lambda_{n_w}(Y - \E[Y]) \geq -\beta] \geq 1-\delta,
    \end{equation*}
    with $\beta = r_z^2 \nrm{\ten{M}}_2^2 \sqrt{2\nsample \ln(2 n_w /\delta)}$. Hence,
    \begin{equation*}
        \lambda_{n_w}(Y) \geq \lambda_{n_w}(\E[Y]) - \beta \geq \nsample \lambda_{n_w}(\E[Y_i])  - \beta.
    \end{equation*}
    So $\nrm{Y^{-1}}_2 = \lambda_1(Y^{-1}) \leq (\nsample \lambda_{n_w}(\E[Y_i]) - \beta)^{-1}$, with probability at least $1-\delta$. 
    Here we used a.s. invertibility of $Y$ for $N \geq n_w$, which follows by \cref{cor:nondeg}. 
    Using this fact, $\nrm{H_i}_2 \leq \nrm{Y^{-1}}_2 \nrm{Y_i}_2$ and the definition of $\zeta_{\mean}$ completes the proof. 
\end{proof}
\begin{remark} \label{rem:zeta-mean}
    We can use \cref{lem:mean-sample-complexity} to tune the way we construct samples $z$. We cannot affect $\nrm{\op{Z}}_2^2$ and $\tau_{\mean}$,
    since they only depend on $\ten{M}$. Only $\gamma_{\mean}$, which ideally is as large as possible, depends on the distribution of $z$. 
    Note that $r_z$ does not directly affect the bound and we want $z$ to be as spread out as possible within its support.
\end{remark}

==> content/identification/old/smoment-bounds.tex <==
% Similarly to mean estimation, we derive a confidence interval centered around $\cmomenth$ defined above.

% \paragraph{Data-driven bound} We again consider the zero-mean terms in the error model discussed in \cref{sec:persistent}:
% \begin{equation*}
%     \svec(\cmoment - \cmomenth) = \ssum_{i=1}^\nsample \opm{H}_i \svec(E_i),
% \end{equation*}
% with $\opm{H}_i \dfn \pinv{(\ssum_{i=1}^{\nsample} \trans{\op{Z}_\kron}(z_i) \op{Z}_\kron(z_i))} \trans{\op{Z}_\kron}(z_i) \op{Z}_\kron(z_i)$
% and the corresponding linear operators $\op{H}_i$. So, under \cref{asm:pe}, the error is given by a sum of norm-bounded zero-mean independent random matrices $\op{H}_i(E_i)$. 
% Here independence follows by \cref{asm:data}. Note that $-W \sleq E_i \sleq w_i \trans{w_i}$ implies $\nrm{E_i}_2 \leq r^2$. Hence, from \cref{lem:mathfd}, with $[\gamma]_i = \nrm{\op{H}_i}_2 r^2$
% \begin{lemma} \label{lem:cmoment-dd}
%     Following the setup of \cref{sec:state-meas} and \cref{asm:data}--\ref{asm:pe} with $N \geq N_0$. 
%     Let $\cmomenth = \pinv{\opm{Z}}_{\cmoment} Y_{\cmoment}$ and $\zeta^2_{\cmoment} \dfn \ssum_{i=1}^N \nrm{\op{H}_i}_2^2$. Then,
%     \begin{equation*}
%         \prob[\nrm{\cmoment - \cmomenth}_2 \leq \beta_{\cmoment}] \geq 1-\delta,
%     \end{equation*}
%     with $\beta_{\cmoment} = r^2 \zeta_{\cmoment} \sqrt{2 \ln(2n_w/\delta)}$.
% \end{lemma}

% \paragraph{Sample complexity}
% Similar to before we study how $\zeta_{\cmoment}$ depends on $\nsample$.
% \begin{lemma} \label{lem:cmoment-sample-complexity}
%     We follow \cref{def:ls-est} and \cref{asm:data}--\ref{asm:pe} with $N \geq \sd{n_z}$ 
%     and assume additionally that $\nrm{z_i}_2 \leq r_z$ a.s. for all $i \in \N_{1:N}$. Then, if $N \geq (r_z^2 \nrm{\op{Z}}_2^2 \tau_{\cmoment}/\lambda_{d_{\cmoment}}(\E[\trans{\op{Z}_{\otimes}} \op{Z}_{\otimes}]))$,
%     \begin{equation*}
%         \prob\left[\zeta_{\cmoment} \leq \frac{
%                 n_w r_z^2 \nrm{\op{Z}}_2^2}{
%                 \sqrt{N} \lambda_{d_{\cmoment}}(\E[\trans{\op{Z}_{\otimes}} \op{Z}_{\otimes}]) - r_z^2 \nrm{\op{Z}}_2^2 \tau_{\cmoment}}
%         \right] \leq \delta,
%     \end{equation*}    
%     with $\tau_{\cmoment} \dfn \sqrt{2\ln(2d_{\cmoment}/\delta)}$ 
%     and $d_{\cmoment} = \rk(\ten{W}_{(1)})$.
% \end{lemma}
% \begin{proof}
%     We closely follow the proof of \cref{lem:mean-sample-complexity}.
%     Let $U \in \Re^{\sd{n_w} \times d_{\cmoment}}$ denote an orthogonal matrix whose columns span $\img(\ten{W}_{(1)})$. 
%     From similar arguments as the one in \cref{lem:mean-sample-complexity}, while using \cref{cor:rank-kron-condition} instead of \cref{lem:rank-condition},
%     gives $\lambda_i(\trans{\opm{Z}_{\cmoment}} \opm{Z}_{\cmoment}) = \lambda_i(\trans{U} \trans{\opm{Z}_{\cmoment}} \opm{Z}_{\cmoment} U)$ 
%     for all $i \in \N_{1: d_{\cmoment}}$ and $\lambda_i(\E[\trans{\op{Z}_{\kron}} \op{Z}_{\kron}]) = \lambda_i(\trans{U} \E[\trans{\op{Z}}_{\kron} \op{Z}_{\kron}] U)$

%     For all $i \in \N_{1:N}$, let $\opm{Y}_i \dfn \trans{\opm{U}}( \trans{Z_i} Z_i \skron \trans{Z_i} Z_i) \opm{U}$,
%     $\opm{D}_i \dfn \opm{Y}_i - \E[\opm{Y}_i]\in \sym{r}$ and $\opm{Y} \dfn \ssum_{i=1}^{\nsample} \opm{Y}_i$. 

%     Note that $\E[\opm{Y}_i] = \trans{\opm{U}} \E[\trans{\op{Z}_{\otimes}} \op{Z}_{\otimes}] \opm{U}$. 
%     Moreover $\nrm{\opm{Y}_i}_2 \leq r_z^2 \nrm{\trans{\op{Z}_{\otimes}} \op{Z}_{\otimes}}_2 \leq r_z^2 \nrm{\op{Z}}_2^2$ (cf. \cref{lem:zopnorm}) and
%     $\nrm{\opm{D}_i}_2 \leq r_z^2 \nrm{\op{Z}}_2^2$. A direct application of \cref{lem:mathfd} gives
%     \begin{equation*}
%         \prob[\lambda_{d_{\cmoment}}(\opm{Y} - \E[\opm{Y}]) \geq -\beta] \leq \delta,
%     \end{equation*}
%     with $\beta = r_z^2  \nrm{\op{Z}}_2^2 \sqrt{2N\ln(2d_{\cmoment}/\delta)}$ and we used $\lambda_{d_{\cmoment}}(\opm{Y} - \E[\opm{Y}]) =
%     \lambda_{d_{\cmoment}}(\ssum_{i=1}^\nsample \opm{D}_i)$. Hence,
%     \begin{equation*}
%         \lambda_{d_{\cmoment}}(\opm{Y}) \geq \lambda_r(\E[\opm{Y}]) - \beta \geq N \sigma_r^2(\E[\op{Z}_{\otimes}]) - \beta. 
%     \end{equation*}
%     Therefore $\nrm{\pinv{\opm{Y}}}_2 = \lambda_1(\pinv{\opm{Y}}) \leq (N \lambda_{d_{\cmoment}}(\E[\trans{\op{Z}_{\otimes}} \op{Z}_{\otimes}]))- \beta)^{-1}$,
%     with probability at least $1-\delta$. From \cref{lem:sopbnd}, $\nrm{\op{H}_i}_2 \leq n_w \nrm{\pinv{\opm{Y}} }_2 \nrm{\opm{Y}_i}_2$.
%     Substituting into the definition of $\zeta_{\cmoment}$ completes the proof. 
% \end{proof}
% \begin{remark}
%     Some of the intuition behind \cref{rem:zeta-mean} generalizes to estimation of $\cmoment$, although the value of 
%     $\sigma_{d_{\cmoment}}^2(\E[\op{Z}_{\otimes}])$ is less intuitive. From \cref{lem:zopprop:d} is it clear that 
%     we want the values of $[\Xi]_{ij}$ to be larger for larger minimum singular values of $[\ten{M}]_{:j:} \skron [\ten{M}]_{:i:}$,
%     although due to the approximations in the proof of \cref{lem:cmoment-sample-complexity} this is not an exact argument. 
% \end{remark}


Similarly to mean estimation, we derive a confidence interval centered around $\cmomenth$ defined above. We also derive radii depending directly on $N$. 

\paragraph{Data-driven bound} Similarly to before, we consider now the zero-mean terms:
\begin{equation*}
    \svec(\cmoment - \cmomenth) = \ldots +  \ssum_{i=1}^{\nsample} \opm{H}_i \svec(E_i),
\end{equation*}
with $\opm{H}_i \dfn \pinv{(\ssum_{j=1}^{\nsample} \trans{\op{Z}_{\kron}}(z_j) \op{Z}_{\kron}(z_j))} \trans{\op{Z}_{\kron}}(z_i) \op{Z}_{\kron}(z_i)$.
Similarly to the mean case:
\begin{proposition} \label{lem:cmoment-dd}
    We follow \cref{def:ls-est} and \cref{asm:data}--\ref{asm:nondeg-cmoment} with $N \geq n_z$. 
    Let $\cmomenth = \pinv{\opm{Z}_{\cmoment}} Y_{\cmoment}$ and $\zeta^2_{\cmoment} \dfn \ssum_{i=1}^N \nrm{\op{H}_i}_2^2$. Then,
    \begin{equation*}
        \prob[\nrm{\cmoment - \cmomenth}_2 \leq \beta_{\cmoment}] \geq 1-\delta,
    \end{equation*}
    with $\beta_{\cmoment} = r^2 \zeta_{\cmoment} \sqrt{2 \ln(2n_w/\delta)}$.
\end{proposition}
\begin{proof}
    Under \cref{asm:nondeg-cmoment}, by \cref{cor:nondeg-cmoment}, 
    the error is given by a sum of norm-bounded zero-mean independent random matrices $\op{H}_i(E_i)$ (with $\opm{H}_i$ the matrix of $\op{H}_i$). 
    Here independence follows by \cref{asm:data}. Note that $-W \sleq E_i \sleq w_i \trans{w_i}$ implies $\nrm{E_i}_2 \leq r^2$. 
    Hence, from \cref{lem:mathfd}, with $[\gamma]_i = \nrm{\op{H}_i}_2 r^2$ we get the required result. 
\end{proof}

\paragraph{Sample complexity} 
Again, by independence, we can expect that $\zeta_{\cmoment}$ decreases with $1/\sqrt{N}$.
We formalize this in a simplified setting.
\begin{lemma} \label{lem:cmoment-sample-complexity_}
    We follow \cref{def:ls-est} and \cref{asm:data}--\ref{asm:nondeg-cmoment} with $N \geq n_z$
    and assume additionally that $V = I$ and $\nrm{z_i}_2 \leq r_z$ a.s. for all $i \in \N_{1:N}$. Then, if  $N \geq (\nrm{\ten{M}}_2^4 \tau_{\cmoment}/ \gamma_{\cmoment})^2$,
    \begin{equation*}
        \prob\left[\zeta_{\cmoment} \leq \frac{\nrm{\ten{M}}_2^4}{\sqrt{N} \gamma_{\cmoment} - \nrm{\ten{M}}_2^4 \tau_{\cmoment}}\right] \leq \delta,
    \end{equation*}    
    with $d_{\cmoment} = \rk(\ten{W}_{(1)})$, $\tau_{\cmoment} \dfn \sqrt{2\ln(2 d_{\cmoment}/\delta)}$
    and \[\gamma_{\cmoment} \dfn \lambda_{d_{\cmoment}}\left[\ten{W}_{(1)} \left({\E[z \trans{z} \otimes z \trans{z}]}/{r_z^4} \otimes I\right) \trans{\ten{W}}_{(1)}\right],\]
    with $\ten{W} = \ten{M} \skron \ten{M}$. 
\end{lemma}
\begin{proof}
    To deal with non-invertibility issues, we introduce $U \in \Re^{n_w \times d_{\mean}}$, a unitary matrix whose columns span $\img(\ten{W}_{(1)})$.
    For all $i \in \N_{1:\nsample}$, we consider the i.i.d. random matrices $Y_i = \trans{U} \trans{\op{Z}_\kron}(z_i) \op{Z}_\kron(z_i) U$
    and $Y = \ssum_{i=1}^{\nsample} Y_i$. 
    
    By \cref{asm:data}, \cref{cor:rank-kron-condition} and \cref{eq:opzcmoment-stacked}: $\img(\opm{Z}_\cmoment) = \img(\ten{W}_{(3)})$. 
    So $\lambda_{d_\cmoment}(Y) = \lambda_{d_\cmoment}(\trans{U} \trans{\opm{Z}_\cmoment} \opm{Z}_{\cmoment} U) = \lambda_{d_\cmoment}(\trans{\opm{Z}_\cmoment} \opm{Z}_{\cmoment})$. 
    Moreover $Y \sgt 0$. Similarly $\E[\trans{\op{Z}_{\kron}} \op{Z}_{\kron}] = \ten{W}_{(1)} (\E[(z \skron z) \trans{(z \skron z)}] \kron I) \trans{\ten{W}_{(1)}}$,
    with $\E[(z \skron z) \trans{(z \skron z)}] \sgt 0$ by \cref{asm:data} and \cref{cor:rank-kron-condition}. So $\lambda_{d_\cmoment}(\E[Y_i]) = \lambda_{d_\cmoment}(\E[\trans{\op{Z}_{\kron}} \op{Z}_{\kron} ])$.
    
    Moreover, since $U$ is unitary, $\nrm{{Y}_i}_2 \leq r_z^2 \nrm{\trans{\op{Z}_{\otimes}} \op{Z}_{\otimes}}_2 \leq r_z^2 \nrm{\ten{M}}_2^4$ (cf. \cref{lem:zopnorm}).
    
    The rest of the proof is identical to that of \cref{lem:mean-sample-complexity}, applied to this selection of $Y_i$.

    % Let $U \in \Re^{n_w \times d_{\mean}}$ denote an orthogonal matrix whose columns span $\img(\ten{M}_{(1)})$.
    % We will be using the deterministic matrix $U$ to restrict the vector space over which we operate.
    % This enables us to deal with the pseudoinverse in the concentration inequalities. To do so we need to consider its 
    % effect on $\trans{\opm{Z}_{\mean}} \opm{Z}_{\mean}$ and $\E[\trans{\op{Z}} \op{Z}]$, which we do through \cref{lem:rank-convergence}. 

    % By \cref{lem:rank-convergence} and \cref{asm:data}--\ref{asm:pe} we know that $\row(\opm{Z}_{\mean}) = \img(\ten{M}_{(1)})$ a.s. 
    % So all eigenvectors related to non-zero eigenvalues of $\trans{\opm{Z}_{\mean}} \opm{Z}_{\mean}$ are in $\img(\ten{M}_{(1)})$.
    % Therefore $\lambda+{d_{\mean}}(\trans{\opm{Z}_{\mean}} \opm{Z}_{\mean}) = \lambda_{d_{\mean}}(\trans{U} \trans{\opm{Z}_{\mean}} \opm{Z}_{\mean} U)$ 
    % for all $i \in \N_{1: d_{\mean}}$. 

    % Note that, by \cref{lem:zopexp:a}, $\E[\trans{\op{Z}} \op{Z}] = \ten{M}_{(1)} (\E[z \trans{z}] \otimes I) \trans{\ten{M}_{(1)}}$. 
    % By \cref{lem:rank-condition} and \cref{asm:data}--\ref{asm:pe}, $\E[z \trans{z}] \sgt 0$. Hence, by \cite[Thm.~4.2.15]{Horn1991} $(\E[z \trans{z}] \otimes I) \sgt 0$. 
    % Therefore $\lambda_{d_{\mean}}(\E[\trans{\op{Z}} \op{Z}]) = \lambda_{d_{\mean}}(\trans{U} \E[\trans{\op{Z}} \op{Z}] U)$.

    % We are now ready for the main part of the proof. 
    % For all $i \in \N_{1:\nsample}$, consider the i.i.d. random matrices $Y_i = \trans{U} \trans{\op{Z}}(z_i) \op{Z}(z_i) U$, $\Delta_i = Y_i - \E[Y_i]$ 
    % and $Y \dfn \ssum_{i=1}^{\nsample} Y_i$. 
    % We have $\E[Y_i] = \trans{U} \E[\trans{\op{Z}} \op{Z}] U$
    % and $\nrm{Y_i}_2 \leq r_z \nrm{\op{Z}}_2^2$ . Since $-r_z \nrm{\op{Z}}_2^2 I \sleq -\E[Y_i] \sleq \Delta_i \sleq Y_i \sleq r_z^2 \nrm{\op{Z}}_2^2 I$,
    % we have $\nrm{\Delta_i}_2 \leq r_z^2 \nrm{\op{Z}}_2^2 \leq r_z^2 \nrm{\ten{M}}_2$ (cf. \cref{lem:zopnorm}). A direct application of \cref{lem:mathfd} gives
    % \begin{equation*}
    %     \prob[\lambda_{ d_{\mean}}(Y - \E[Y]) \geq -\beta] \geq 1-\delta,
    % \end{equation*}
    % with $\beta = r_z^2 \nrm{\ten{M}}_2 \sqrt{2\nsample \ln(2 d_{\mean} /\delta)}$. Hence,
    % \begin{equation*}
    %     \lambda_{ d_{\mean}}(Y) \geq \lambda_{ d_{\mean}}(\E[Y]) - \beta \geq \nsample \lambda_{ d_{\mean}}(\E[Y_i])  - \beta.
    % \end{equation*}
    % So $\nrm{\pinv{Y}}_2 = \lambda_1(\pinv{Y}) \leq (\nsample \lambda_{  d_{\mean}}(\E[Y_i]) - \beta)^{-1}$, with probability at least $1-\delta$. 
    % Using this fact, $\nrm{H_i}_2 \leq \nrm{\pinv{Y}}_2 \nrm{Y_i}_2$ and the definition of $\zeta_{\mean}$ completes the proof. 
\end{proof}
\begin{remark} \label{rem:zeta-cmoment}
    The behaviour of $\zeta_{\cmoment}$ as described by \cref{lem:cmoment-sample-complexity} is very similar to that of $\zeta_{\mean}$. 
    The main difference is that $\gamma_{\cmoment}$ now depends on the kurtosis of $z$ (i.e. the fourth order moment). Still, we see that 
    it does not depend on $r_z$ directly. Only the spread of $z \otimes z$ within its support affects it. 
\end{remark}

==> content/identification/old/state-measurements.tex <==
We assume access to independent state samples. That is a sequence $\{(y_i, z_i)\}_{i\in \N_{1:\nsample}}$, satisfying 
\begin{equation} \label{eq:affmodel}
    y_i = \tucker{\hm{\ten{M}}; z_i, (w_i, 0)} = \tucker{\ten{M}; z_i, w_i},
\end{equation}
with $\{z_i\}_{i\in \N_{1:\nsample}}$ a sequence of independent random vectors and $\ten{M} \dfn [\hm{\ten{M}}]_{:,:,1:n_w} \in \Re^{n_x \times n_z \times n_w}$.  


Moreover, to guarantee an equivalent of \emph{persistent excitation}, we assume that the support of $z_i$ is not degenerate
as is formalized in the following assumption.
\begin{assumption} \label{asm:data_}
    We assume that $\{z_i\}_{i\in\N_{1:\nsample}}$ is a sequence of i.i.d. copies of a random vector $z$,
    with a distribution that is dominated by the Lebesgue measure.
\end{assumption}
\begin{remark} \label{rem:asm_}
    Independence is guaranteed by either \emph{(i)} taking a known random 
    $z_i = (x_0, u_0)$, updating \eqref{eq:dyn} once and taking $y_i = x_1 - {[\hm{\ten{M}}]_{::\nwh:}} z_i$; or \emph{(ii)} 
    taking a known $x_0$, updating \eqref{eq:dyn} $T$ times for random $u_t$ and taking $y_i = x_T- {[\hm{\ten{M}}]_{::\nwh}} z_i$ and $z_i = (x_{T-1}, u_{T-1})$.\todo{ctrb and $\Xi$?} 
    We refer to \emph{(ii)} as \emph{rollout (r.o.)} as in \cite{Xing2020, Dean2019}
    and to \emph{(i)} as \emph{random initialization (r.i.)}. 
\end{remark}

The data follows a bilinear model. Specifically, $\forall i \in \N_{1:\nsample}$,
\begin{align}
    {y}_i &= \op{Z}(z_i) {w}_i, \quad \text{with } \op{Z} \colon z \mapsto (\ten{M} \btimes{2} z).\label{eq:linearmodel}
\end{align}

Besides $\op{Z}(z)$ consider the operator,
\begin{equation} \label{eq:Zkron}
    \op{Z}_{\kron} \colon z \mapsto {\op{Z}(z)} \skron {\op{Z}(z)}.
\end{equation}
We list more convenient forms of these operators in \cref{lem:zopeq}.

\begin{remark} \label{rem:basis}
    The true $\ten{M}$ might be unknown, so one should be selected such that \eqref{eq:linearmodel} holds. We call such a $\ten{M}$ a \emph{basis} for estimation. 
    If $n_w = n_x n_z$ and $[\ten{M}]_{::i}$ are linearly independent, we call the basis \emph{model-free}. Then we can model any dynamics \eqref{eq:dyn}
    ($[A(w), B(w)] = \ssum_{i=0}^{\nwh} {[\ten{M}]_{::i}} [w]_i$),
    by selecting a suitable distribution $w$. Hence \eqref{eq:linearmodel} is always satisfied.  
\end{remark}

By \eqref{eq:modendef}, $\op{Z}(z)$ is a weighted sum of matrices. Thus studying invertibility of $\op{Z}(z)$ is analogous to invertibility of a linear subspace of matrices (or linear forms),
which is an unsolved problem in general (cf. \cite{Testa2018} for $3 \times 3$ matrices).
We consider the following result \cite{Lovasz1989}.
\begin{proposition}
    Let $z$ denote a random vector with non-degenerate support (cf. \cref{asm:data})
    and $n_x \geq n_w$. Then, $\op{Z}(z)$ is left invertible either with probability one or zero. 
\end{proposition}
This suggests that it is often sufficient to sample $\op{Z}(z)$ for one random $z$ and check its invertibility. The conclusion will then 
generalize with probability one. When successful, we can determine ${w}_i$ exactly based on ${y}_i$ 
and \cref{lem:dd-moment} is applicable. 

We however also want to estimate $\mean$ and $\cmoment$ in the other case (i.e., when $n_x < n_w$). For example, for a model-free basis (cf. \cref{rem:basis}) we have $n_w = n_x n_z > n_x$.  
To do so we design least squares estimators. 

Note that \eqref{eq:linearmodel} directly leads to two linear models. One for the mean and one for the second moment. 
Specifically the dependency between the data and the mean is: 
\begin{equation} \label{eq:errmodel-mean}
    y_i = \op{Z}(z_i) (\mean + \epsilon_i), 
\end{equation}
with $\epsilon_i \dfn w_i - \mean$ a zero-mean error term.

Using \eqref{eq:skronfund}, the second moment data model is:
\begin{align}
    y_i \skron y_i = \op{Z}_{\kron}(z_i) ( \svec(\cmoment) +  \svec(E_i)), \label{eq:errmodel}
\end{align}
with $E_i \dfn {w}_i \trans{{w}_i} - \cmoment$ zero-mean i.i.d. random matrices.

We introduce two least-squares (LS) estimators:
\begin{definition} \label{def:ls-est}
    Consider models \cref{eq:errmodel-mean,eq:errmodel}. Then:
    \begin{enumerate}
        \item Let $Y_{\mean} \dfn (y_1; \dots; y_\nsample)$ and $\opm{Z}_{\mean} \dfn [\op{Z}(z_1); \dots; \op{Z}(z_\nsample)]$.
                The \emph{mean LS estimator} is then $\meanh = \pinv{\opm{Z}_{\mean}} Y_{\mean}$. 
        \item Let $Y_\cmoment = [y_1 \skron y_1; \dots; y_\nsample \skron y_\nsample]$ and $\opm{Z}_\cmoment = [\op{Z}_{\kron}(z_1); \dots; \op{Z}_{\kron}(z_\nsample)]$.
                The \emph{second moments LS estimator} is then $\cmomenth = \unsvec(\pinv{\opm{Z}}_{\cmoment} Y_{\cmoment})$. 
    \end{enumerate}
\end{definition}
A similar estimator to $\cmomenth$ is used in compressed covariance sensing \cite{Romero2013}, where 
it is observed that it acts as a good heuristic for the \emph{maximum likelihood estimator} when $w$ is Gaussian. Noting that each element of the vector
equation \eqref{eq:errmodel} constitutes a bilinear form of $z_i$, reveals a connection with bilinear estimation \cite{Kukush2003}. There adjusted LS
estimators exist that are consistent even when $z_i$ is perturbed by random noise. For simplicity we consider exact state measurements here, 
which enables the use of ordinary LS, for which it is convenient to derive concentration inequalities. 

The performance of the estimators $\meanh$ and $\cmomenth$ is analyzed next. Before doing so we comment on estimator bias.

==> content/structure/lqr.tex <==
The goal of this section is twofold \emph{(i)} we argue how LQ control of CP dynamics is equivalent 
to \cref{eq:slqr}; and \emph{(ii)} we show how the optimal policy is determined by solving a SDP,
generalizing the result of \cite{Balakrishnan2003}.  

We start by stating the CP equivalent of \cref{eq:slqr}
\begin{equation} \label{eq:lqrcp}
    \begin{alignedat}{2}
        &\minimize_{Z_t} &\quad& \sum_{t=0}^\infty \tr[Z_t H] \\
                             &\stt && Z_t = \begin{bmatrix}
                                 X_t & V_t \\ \trans{V_t} & U_t
                             \end{bmatrix} \sgeq 0, \\&&&X_{t+1} = \op{E}(Z_t), \quad \forall t \in \N,
    \end{alignedat} \tag{$\mathcal{LQR}_{\mathrm{cp}}$}
\end{equation}
with $H \dfn \blkdiag(Q, R) \sgt 0$. The psd. constraint on $Z_t$ ensures that it acts 
like the second moment of a random vector. 

% It is well known that the optimal policy for \eqref{eq:slqr} is linear: $u_t = K_\star x_t$ 
% for some $K_\star \in \Re^{n_u \times n_x}$ \cite{Coppens2019,Morozan1983}. 
% Selecting $H = \blkdiag(Q, R)$ and, as before, letting $X_t = \E[x_t \trans{x_t}]$, $U_t = \E[u_t \trans{u_t}] = K_\star X_t \trans{K}_\star$ 
% and $V_t = \E[x_t \trans{u_t}] = X_t \trans{K}_\star$ and using \cref{eq:dynsm_} shows that \eqref{eq:lqrcp} lower bounds 
% the cost of \cref{eq:slqr}. In fact, we can prove the stronger res:
We show that \eqref{eq:slqr} is equivalent to \eqref{eq:lqrcp}
\begin{proposition} \label{thm:cpmulteq}
    Let $\mathrm{Val}(\cdot)$ denote the optimal value. Then 
    \begin{equation*}
        \mathrm{Val}\eqref{eq:slqr} = \mathrm{Val}\eqref{eq:lqrcp},
    \end{equation*}
    given \cref{asm:model}. Moreover sequence $(Z_t)_{t \in \N}$ is feasible for \eqref{eq:lqrcp} iff there is a feasible sequence
    in \eqref{eq:slqr} $u_t = K_t x_t + \delta_t$ s.t.
    $Z_t = \E[z_t \trans{z_t}]$ where $z_t = (x_t, u_t)$. 
    Here $K_t \in \Re^{n_x \times n_u}$
    and $\delta_t \in \Re^{n_u}$ is a random vector $\forall t \in \N$.
\end{proposition}
\begin{proof}
    Deferred to Appendix~\ref{app:lqr}.
\end{proof}

To find the exact solution of \eqref{eq:lqrcp}, similarly 
to usual LQR, we need to consider a Riccati equation:
\begin{equation} \label{eq:ric-def}
    \op{R}(P) \dfn Q + \adj{\op{F}}(P) - \trans{(\adj{\op{H}})}(P)(R + \adj{\op{G}}(P))^{-1}\adj{\op{H}}(P).
\end{equation}
where $\adj{\op{F}}(P) = \ten{A}_{(2)} (\smoment \kron P) \trans{\ten{A}_{(2)}}$, 
$\adj{\op{G}}(P) = \ten{B}_{(2)} (\smoment \kron P) \trans{\ten{B}_{(2)}}$ and 
$\adj{\op{H}}(P) = \ten{B}_{(2)}(\smoment \otimes P) \trans{\ten{A}_{(2)}}$ with tensors $\ten{A}$ and $\ten{B}$ 
as in \cref{eq:dynten}. We use adjoint CP operators to be consistent with \cref{cor:cpadj}.

\begin{remark}
    The operators $\adj{\op{F}}$, $\adj{\op{H}}$ and $\adj{\op{G}}$ form
    the blocks of $\adj{\op{E}}$ when it is partitioned similarly to $Z_t$ (cf. \cref{lem:opadj}). 

    In the deterministic setting with $n_w = 1$ and $w_t = 1$ (so $\E[W] = 1$), we have $\adj{\op{F}}(P) = \trans{A}_1 P A_1$, $\adj{\op{H}}(P) = \trans{B}_1 P A_1$ and $\adj{G}(P) = \trans{B}_1 P B_1$.
    Hence we recover the classical Riccati operator as a special case. 
\end{remark}

We introduce the \emph{closed-loop operators} as
\begin{equation} \label{eq:clops}
    \Pi_K(X) \dfn [I; K] X [I, \trans{K}], \, \op{E}_K(X) \dfn \op{E}(\Pi_K(X)),
\end{equation}
The policy $Z_t = \Pi_K(X_t)$ is recovered when taking $u_t = Kx_t$ 
in the equivalent \eqref{eq:slqr} (cf. \cref{thm:cpmulteq}).

We can then state the following theorem.

\begin{theorem} \label{thm:cplqr}
    \shorten*{Let $\exists K\colon \rho(\op{E}_K) < 1$ and $H \dfn \blkdiag(Q, R) \sgt 0$.} Then 
    $Z_t = \Pi_{K_{\star}}(X_t)$ is \update*{an} optimal policy, 
        with $K_{\star} = -(R + \adj{\op{G}}(P_{\star}))^{-1} \adj{\op{H}}(P_{\star})$ and $P_{\star} \sgt 0$
        solves the Riccati equation $P_{\star} = \op{R}(P_\star)$. Moreover
    \begin{enumerate}
        \item \label{thm:cplqr:b} $\rho(\op{E}_{K_\star}) < 1$; 
        \item $\mathrm{Val}\eqref{eq:lqrcp} = \tr[P_{\star} X_0]$;
        % \item \label{thm:cplqr:d} $P_\star  \in \argmax \left\{\tr[P X_0] \colon \adj{\op{L}}(P) \sleq H, P \sgeq 0 \right\}$.\\
        %                                     The solution to this SDP is unique if $X_0 \sgt 0$. 
    \end{enumerate}
\end{theorem}
\begin{proof}
    \ilarxiv{See Appendix~\ref{app:lqr} for the full proof.}\ilpub{This result was shown for multiplicative noise in \cite{Coppens2019, Morozan1983} 
    and generalized to the CP setting by \cref{thm:cpmulteq}. Nonetheless, a full proof is included in the technical report \citear{}.}
\end{proof}

\begin{prepupdate}
    \begin{remark} \label{rem:stabilizability}
        Here $\exists K \colon \rho(\op{E}_K(\cdot)) < 1$ 
        is referred to as \emph{stabilizability}. Among other things 
        it implies the system being below the \emph{uncertainty threshold} \cite{Athans1977}.
    \end{remark}
\end{prepupdate}

\begin{arxiv}
    \begin{example}
        Let us consider a deterministic system with $n_w = 1$ and
        \begin{equation*}
            A_1 = \begin{bmatrix}
                1 & 0.1 \\ 
                0 & 1
            \end{bmatrix}, \, B_1 = \begin{bmatrix}
                0 \\ 0.1
            \end{bmatrix}.
        \end{equation*}
        This will help us understand how \cref{eq:lqrcp} generalizes the usual notions of LQR. We pick $H = \diag(1, 1, 0.1)$. Then 
        the solution described by \cref{thm:cplqr} is approximately:
        \begin{equation*}
            K = [-1.75, -2.64].
        \end{equation*}
        One can easily verify that this is the usual LQR solution in the deterministic setting. Let's spend some time noting what happens when 
        we set $X_0 = x_0 \trans{x_0}$. In that case, for some $u_0$, let $Z_0 = (x_0, u_0) \trans{(x_0, u_0)}$. Then (similarly to \cref{ex:smdyn}):
        \begin{align*}
            \op{E}(Z_0) &= A_1 x_0 \trans{x_0} \trans{A}_1 + A_1 x_0 \trans{u_0} \trans{B_1} \\ &\qquad + B_1 u_0 \trans{x_0} \trans{A}_1 + B_1 u_0 \trans{u_0} \trans{B_1}.
        \end{align*}
        It is not difficult to verify that this equals $x_1 \trans{x_1}$ for $x_1 = A_1 x_0 + B_1 u_0$. We could repeat this for each time step 
        noting that $X_t = x_t \trans{x_t}$ and $Z_t = (x_t, u_t) \trans{(x_t, u_t)}$ in \cref{eq:lqrcp}. Trivially we have $Z_t \sgeq 0$,
        so the trajectory is feasible. Moreover the cost becomes $\tr[Z_t H] = \trans{x_t} I x_t + 0.1 \trans{u_t} I u_t$. So we can see 
        that the classical LQR controller is at least a feasible solution to \cref{eq:lqrcp} where we then have 
        \begin{align*}
            Z_t = \Pi_K(X_t) &= \begin{bmatrix}
                x_t \trans{x_t} & x_t \trans{x}_t \trans{K} \\ K x_t \trans{x_t} & K x_t \trans{x}_t \trans{K}
            \end{bmatrix} \\ &= (x_t, Kx_t) \trans{(x_t, Kx_t)}.
        \end{align*}
        Note that we have shown in \cref{thm:cplqr} that such policies are in fact optimal. In terms of classical LQR this 
        implies that, a random policy $u_t = Kx_t + \delta_t$ for some random $\delta_t$ will not improve performance. 
    \end{example}
\end{arxiv}

% We are specifically interested in the case $N \to \infty$. 
% \begin{theorem} \label{thm:_cplqr}
%     Consider \eqref{eq:lqr-finite}. Assume $\exists K\colon \rho(\op{E}_K) < 1$ and $H \sgt 0$. Then
%     the optimal policy is $Z_t = \Pi_{K_{\star}}(X_t)$, 
%         with $K_{\star} = -(R + \adj{\op{G}}(P_{\star}))^{-1} \adj{\op{H}}(P_{\star})$ and $P_{\star} \sgt 0$
%         solves the Riccati equation $P_{\star} = \op{R}(P_\star)$. Moreover
%     \begin{enumerate}
%         \item \label{thm:_cplqr:b} $\rho(\op{E}_{K_{\star}}) < 1$; 
%         \item $\op{J}^\star(X_0) = \tr[P_{\star} X_0]$;
%         \item \label{thm:_cplqr:d} $P_\star  \in \argmax \left\{\tr[P X_0] \colon \adj{\op{L}}(P) \sleq H, P \sgeq 0 \right\}$.\\
%                                             The solution to this SDP is unique if $X_0 \sgt 0$. 
%     \end{enumerate}
%     Here $\op{L}(Z)$ is as defined in \cref{eq:lyapdef}. The operators $\adj{\op{F}}, \adj{\op{G}}$ and $\adj{\op{H}}$ 
%     are as in \cref{eq:ope-partition}. 
% \end{theorem}
% \begin{proof}
%     See the proof in Appendix~\ref{app:lqr}.
% \end{proof}
% \begin{remark}
%     The uniqueness result \cref{thm:cplqr:d} indicates the need for regularization. That is, instead of taking $X_0 = x_0 \trans{x_0}$
%     for a deterministic initial state we will consider $X_0 = x_0 \trans{x_0} + \lambda I$ for some small $\lambda > 0$. 
% \end{remark}
% \begin{remark}
%     The constraint of the SDP in \cref{thm:cplqr:d} is
%     \begin{equation*}
%         \begin{bmatrix}
%             Q - P + \ten{A}_{(2)} (\smoment \kron I) \trans{\ten{A}_{(2)}} & \ten{A}_{(2)} (\smoment \kron I) \trans{\ten{B}_{(2)}} \\ 
%             \ten{B}_{(2)} (\smoment \kron I) \trans{\ten{A}_{(2)}} & R + \ten{B}_{(2)} (\smoment \kron I) \trans{\ten{B}_{(2)}}
%         \end{bmatrix} \sgeq 0.
%     \end{equation*}
%     The result is therefore equivalent to that of \cite[Prop.~3]{Coppens2021} and is direct generalization 
%     of the continuous time reformulation of \cite[\S{}V]{Balakrishnan2003} to discrete time when $n_w = 0$. 
% \end{remark}


% One issue with the SDP considered in \cref{thm:cplqr} is that the feasible solutions $P$ will not necessarily lead to
% stabilizing controllers. Therefore, when considering distributionally robust synthesis we will consider the following problem:
% \begin{equation} \label{eq:stab-sdp}
%     \minimize_{(P, K)} \, \{\tr[P X_0] \colon \adj{\op{L}}(K; P) \sgeq \adj{\Pi}(K; H), P \sgeq 0 \},
% \end{equation}
% the constraint of which is a Lyapunov constraint, thereby imposing stability through \cref{prop:lyapcp}. 
% We can show:
% \begin{proposition} \label{prop:stablqr}
%     The problem \eqref{eq:stab-sdp} satisfies:
%     \begin{enumerate}
%         \item \label{prop:stablqr:a} $\rho(\op{E}_K) < 1$ for any feasible $K$;
%         \item $(P_\star, K_{\star})$ is optimal and uniquely so if $X_0 \sgt 0$.
%     \end{enumerate}
% \end{proposition}
% \begin{proof}
%     See the proof in Appendix~\ref{app:lqr}.    
% \end{proof}

Even though we directly tackled second moment dynamics in \cref{thm:cplqr}, 
the optimal policy $Z_t = \Pi_{K_{\star}}(X_t)$ 
is realizable for multiplicative noise dynamics using 
$u_t = K_{\star} x_t$. So this controller is also optimal 
for \eqref{eq:slqr} as is well known (cf. \cite[Prop.~3]{Coppens2019})
and achieves the equality in \cref{thm:cpmulteq}. 

Thus we can conclude that LQR of CP dynamics
is (i) identical to LQR of multiplicative noise dynamics; (ii) 
a natural generalization of classical LQR; and (iii) a relaxation for LQR of 
switching systems in the sense of \cref{thm:stab-eq}. 

The final question is how to find a $P_\star$ satisfying \eqref{eq:ric-def}. Numerical solution 
of such equations is considered in detail in \cite{Damm2003}. We consider a reformulation
as a SDP, akin to \cite{Balakrishnan2003}. 

\begin{theorem} \label{thm:ric-sdp-primal}
    Let $P_\star$ solve the Riccati equation \eqref{eq:ric-def}. Then $P_\star$
    is a maximizer of
    \begin{equation*}
        \begin{alignedat}{2} 
            &\maximize_{P \sgeq 0} &\quad& \tr[P X_0] \\
            &\stt && \begin{bmatrix}
                P - \adj{\op{F}}(P) & -\trans{(\adj{\op{H}})}(P) \\
                -\adj{\op{H}}(P) & -\adj{\op{G}}(P)
            \end{bmatrix} \sleq \begin{bmatrix}
                Q \\ & R
            \end{bmatrix},
        \end{alignedat}
    \end{equation*}
    with $\adj{\op{F}}$, $\adj{\op{H}}$ and $\adj{\op{G}}$ as defined below \eqref{eq:ric-def}. 
    Moreover, when $X_0 \sgt 0$, then $P_\star$ is the unique solution.
\end{theorem}
\begin{proof}
    The proof is analogous to the one in \cite{Balakrishnan2003} and \cite[Prop.~3]{Coppens2019}. \ilarxiv{The full proof is Deferred to Appendix~\ref{app:lqr}.}\ilpub{A full proof in the CP case is Deferred to \citear{}.}
\end{proof}

\update*{When the dynamics are not stabilizable, the SDP in \cref{thm:ric-sdp-primal}
will not have a positive definite solution for $X_0 \sgt 0$.}

==> content/synthesis/old/ambiguity.tex <==
Starting from the ambiguity set constructed in the previous section, we use a synthesis method similar to that of \cite{Coppens2019}. 
That is, we robustify \eqref{eq:stab-sdp}.
To do so we introduce an ambiguity set that combines \cref{lem:mean-dd} and \cref{lem:cmoment-dd}.
\begin{corollary} \label{cor:ambig}
    Following the notation of \cref{lem:mean-dd}, \ref{lem:cmoment-dd}, consider the ambiguity $\amb$ as
    \begin{equation*}
        \{\mu \in \Pf(\W) \colon \nrm{\V_{\mu}[w] - \covarh}_2 \leq \beta_{\covar}, \, \nrm{\E_{\mu}[w] - \meanh}_2 \leq \beta_{\mean}\},
    \end{equation*}
    with $\smomenth = \cmomenth - \meanh \trans{\meanh}$, $\beta_{\mean} = r \zeta_{\mean}(2 + \sqrt{2 \ln(1/\delta_{\mean})})$, $\beta_{\cmoment} = r^2 \zeta_{\cmoment}  \sqrt{2 \ln(2 n_w /\delta_{\cmoment})}$ 
    and $\beta_{\covar} = \beta_{\cmoment} + \beta_{\mean} (\beta_{\mean} + 2 \nrm{\meanh}_2)$. Then $\amb$ satisfies \eqref{eq:amb_conf},
    with $\delta = 1 - \delta_{\cmoment} - \delta_{\mean}$. 
\end{corollary}
\begin{proof}
    From \cref{lem:mean-dd} and \cref{lem:cmoment-dd} we have $\nrm{\mean - \meanh}_2 > \beta_{\mean}$ and $\nrm{\cmoment - \cmomenth}_2 > \beta_{\cmoment}$ 
    with probability under $\delta_{\mean}$ and $\delta_{\cmoment}$ respectively. 
    The definition of $\covarh$ and $\covar = \cmoment - \mean \trans{\mean}$ gives
    \begin{align*}
        &\covar - \covarh = (\cmoment - \cmomenth) - (\mean \trans{\mean} - \meanh \trans{\meanh}).
    \end{align*}
    We can expand the second term as $(\mean - \meanh)\trans{(\mean - \meanh)} + (\mean - \meanh) \trans{\meanh} + \meanh \trans{(\mean - \meanh)}$.
    So, using the Triangle inequality, $\nrm{\covar - \covarh}_2 \leq \nrm{\cmoment - \cmomenth}_2 + \nrm{\mean - \meanh}_2^2 + 2\nrm{\mean - \meanh}_2\nrm{\meanh}_2 = \beta_{\covar}$. 
    Finally $1 - \delta  \geq 1 - \delta_{\covar} - \delta_{\cmoment}$ follows by a union bound. 
\end{proof}

==> content/synthesis/old/complexity.tex <==
We analyze a simpler DR reformulation of \eqref{eq:stab-sdp} next, to quantify the rate of convergence. 
Later this rate is confirmed using numerical experiments. 

Specifically, under the setting of \cref{cor:ambig} we can also consider the following ambiguity set,
\begin{corollary} \label{cor:ambig-smoment}
    Following the notation of \cref{cor:ambig}, then
    \begin{equation*}
        \amb \subseteq \{\mu \in \Pf(\W) \colon \nrm{\E_{\mu}[\hm{w} \trans{\hm{w}}] - \smomenth}_2 \leq \beta_{\smoment}\},
    \end{equation*}
    with $\smomenth = \blkdiag(\covarh, 0) + \op{D}(\meanh)$, $\op{D}$ the dilation operator and $\beta_{\smoment} = \beta_{\cmoment} + \beta_{\mean}(2\beta_{\mean} + 4\nrm{\meanh}_2 + 1)$.
\end{corollary}
\begin{proof}
    Similar to the proof of \cref{cor:ambig} this result follows from a simple triangle inequality:
    \begin{equation*}
       \nrm{\E[\hm{w} \trans{\hm{w}}] - \smomenth}_2 \leq \nrm{\covar - \covarh}_2 + \nrm{\mean \trans{\mean} - \meanh \trans{\meanh}}_2 + \nrm{\op{D}(\mean - \meanh)}_2,
    \end{equation*}
    with $\op{D}$ the dilation operator. 
    From \cref{cor:ambig} we have $\nrm{\covar - \covarh}_2 \leq \beta_{\smoment} = \beta_{\cmoment} + \beta_{\mean}(\beta_{\mean} + 2 \nrm{\meanh}_2)$
    and $\nrm{\mean - \meanh}_2 \leq \beta_{\mean}$. Therefore, by \cite[Eq. 2.1.28]{Tropp2015}, $\nrm{\op{D}(\mean - \meanh)}_2 \leq \beta_{\mean}$
    and, by the arguments in the proof of \cref{cor:ambig}, $\nrm{\mean \trans{\mean} - \meanh \trans{\meanh}}_2 \leq \beta_{\mean}(\beta_{\mean} + 2 \nrm{\meanh}_2)$. 
    This completes the proof. 
\end{proof}

Again considering the ambiguity over second moments, by \cref{cor:ambig-smoment}, $\nrm{\smoment - \smomenth}_2 \leq \beta_{\smoment}$ 
implies $M \in \set{M}$ by \cref{sec:analysis}. Therefore,
by a similar argument to the one used in the proof of \cref{prop:dr-stab-sdp}, a sufficient condition of \eqref{eq:dr-lyap} is:
\begin{equation} \label{eq:dr-lyap-app}
    \op{L}(\smomentdr, K; P) \sleq \adj{\Pi}(K; H),
\end{equation}
with $\smomentdr \dfn \smomenth + \beta_{\smoment} I$. 

Note that \eqref{eq:dr-lyap-app} is identical to
the constraint of \eqref{eq:stab-sdp}, but with $\smomentdr$ instead of $\smoment_{\star}$. 
This motivates the study of:
\begin{equation} \label{eq:stab-sdp-dr-app}
    \minimize_{(P, K)} \,\{\tr[PX_0] \colon P \sgeq 0, \eqref{eq:dr-lyap}\},
\end{equation}
the solution of which satisfies a DR Riccati equation:
\begin{equation*}
    \op{R}(\smomentdr; \bar{P}) = \bar{P}, \quad \bar{K} = -(R + \adj{\op{G}}(\smomentdr; \bar{P}))^{-1} \adj{\op{H}}(\smomentdr; \bar{P}),
\end{equation*}
by direct application of \cref{prop:stablqr} for $\smomentdr$ instead of $\smoment_{\star}$. Here we parametrized 
the involved operators on $\smoment$ as in \cref{sec:synthesis}. 

Since the solution is described by a Riccati equation, we a previous result of the authors \cite{Coppens2020}. Here
the performance of some $\hat{K}$ was compared to that of $K_{\star}$ when the Riccati equation was solved using $\hat{\smoment}$ 
instead of $\smoment_{\star}$ (i.e. the certainty equivalent approach).
In our setting:
\begin{theorem} \label{thm:sample-complexity}
    Let $(\bar{P}, \bar{K})$ achieve the optimum of \eqref{eq:stab-sdp-dr-app}, the assumptions of \cref{lem:mean-sample-complexity,lem:cmoment-sample-complexity} hold
    and $M_{\star} \sgt 0$. Then
    \begin{equation*}
        \tr [\ssum_{t=0}^{\infty} \op{E}^t(\smoment_{\star}, \bar{K}; X_0) \adj{\Pi}(\bar{K}; H)] -  \op{J}^{\star}(X_0) = \op{O}(1/N).
    \end{equation*}
    Here the first term is the closed-loop cost achieved when applying $\bar{K}$ to the true dynamics. 
\end{theorem}
\begin{proof}
    By the assumptions of \cref{lem:mean-sample-complexity,lem:cmoment-sample-complexity}
    and \cref{lem:mean-dd,lem:cmoment-dd}, we have $\beta_{\mean} = \op{O}(1/\sqrt{N})$ 
    and $\beta_{\cmoment} = \op{O}(1/\sqrt{N})$. Based on this one can easily show that, $\beta_{\covar} = \op{O}(1/\sqrt{N})$ by \cref{cor:ambig} and 
    $\beta_{\smoment} = \op{O}(1/\sqrt{N})$ by \cref{cor:ambig-smoment}. 

    Since \cite{Coppens2020} was derived for a relative error bound we will assume $\smoment_{\star} \sgt 0$ for convenience. 
    The results of \cite{Coppens2020} could also be derived for an absolute error bound, which would result in different constants,
    but the same asymptotic rate.

    By \cref{cor:ambig-smoment} we have
    \begin{align*}
        -\beta_{\smoment} I \sleq \smomenth - \smoment \sleq \beta_{\smoment} I \quad  \Leftrightarrow \quad  0 \sleq \smomentdr - \smoment \sleq 2 \beta_{\smoment} I. 
    \end{align*}
    Using the invertibility assumption $2 \beta_{\smoment} I = 2 \beta_{\smoment} \smoment_{\star}^{-1} \smoment_{\star} \sleq 2 \beta_{\smoment} \nrm{\smoment_{\star}^{-1}}_2 \smoment_{\star}$. 
    The resulting bounds satisfy \cite[Asm.~II.2]{Coppens2020}. Applying \cite[Cor.~III.4]{Coppens2020}
    then completes the proof.
\end{proof}

Note that in practice one would never use \cref{eq:stab-sdp-dr-app} to synthesize controllers, since using $\smomentdr$ 
implies $\mu(\W) = \beta_{\smoment} > 1$. Hence $\mu$ is no longer a probability measure. Nonetheless the rate 
$\op{O}(1/N)$ is still optimal even for this conservative overapproximation of \cref{prop:dr-stab-sdp}. One would thus expect 
the less conservative synthesis procedure in \cref{prop:dr-stab-sdp} to achieve a similar rate. This is observed in numerical experiments.
A formal analysis is however outside of the scope of this paper. 

==> content/synthesis/old/synthesis.tex <==
Since we will be varying the second moment we consider $\smoment$ a parameter of the operators introduced in \cref{sec:multiplicative},
similarly to $K$. For example, define $\op{E}_K(W; \cdot) \colon \sym{n_z} \to \sym{n_x}$ as
\begin{equation*}
    \op{E}_K(W; X) = \hm{\ten{M}}_{(3)} (M \otimes \Pi_K(X_t)) \trans{\hm{\ten{M}}}_{(3)}. 
\end{equation*}
Similarly we can define $\op{L}(\smoment, K; X) = X - \op{E}_K(W; X)$. Since $M$ is a parameter and not an argument, 
the adjoints of these operators are the same as the ones of \cref{lem:opadj}. 

Using these explicit parametrizations, we robustify \eqref{eq:stab-sdp} as:
\begin{equation} \label{eq:dr-lyap}
    \adj{\op{L}}(\smoment, K; P) \sgeq \adj{\Pi}(K; P), \quad \forall \smoment \in \set{M},
\end{equation}
with $\set{M} \dfn \{M = \blkdiag(\covar, 0) + \hm{\mean} \trans{\hm{\mean}} \colon \nrm{\mean - \meanh}_2 \leq \beta_{\mean}, \nrm{\covar - \covarh}_2 \beta_{\covar}\}$,
which is the ambiguity set of \cref{cor:ambig} defined over the second moment instead of the measure. As such $\smoment_{\star} \dfn \E_{\mu_{\star}}[\hm{w} \trans{\hm{w}}] \in \set{M}$
with with probability at least $1-\delta$. 

Note that, by switching from $\set{A}$ to $\set{M}$ we ignored the support constraint 
(i.e., $\tr[\covar + \mean \trans{\mean}] \leq r^2$). In practice this effect is minimal, especially since the 
constraint is usually satisfied automatically for large sample counts. 

We will then study the following problem:
\begin{equation} \label{eq:dr-stab-sdp}
    \minimize_{(P, K)} \, \{\tr[X_0P] \colon P \sgeq 0, \eqref{eq:dr-lyap}\}.
\end{equation}



Solving a problem like \eqref{eq:dr-stab-sdp} to approximate the solution of \cref{eq:drlqr} was considered previously 
for DR control in \cite{Coppens2019} and for robust control in \cite{Kothare1996}.
As observed in these references, \eqref{eq:dr-stab-sdp} is not tractable as is. We instead approximate it with an SDP.

Before doing so we generalize \cref{prop:stablqr} to \eqref{eq:dr-stab-sdp}:
\begin{proposition} \label{prop:stablqr-dr}
    Let $\smoment_{\star} \dfn  \E_{\mu_{\star}}[\hm{w} \trans{\hm{w}}]$. Any feasible pair $(P, K)$ of \eqref{eq:dr-stab-sdp} satisfies with probability at least $1-\delta$:
    \begin{enumerate}
        \item $\rho(\op{E}_K(\smoment_{\star}; \cdot)) < 1$;
        \item $\op{J}^\star(X_0) \leq \tr[X_0 P]$. 
    \end{enumerate}
\end{proposition}
\begin{proof}
    By \cref{cor:ambig}, $\prob[\smoment_{\star} \in \set{M}] \geq 1-\delta$. Conditioning on this event means that:
    \begin{equation*}
        \adj{\op{L}}(\smoment_{\star}, K; P) \sgeq \adj{\Pi}(K; H),
    \end{equation*}
    since feasiblity implies \eqref{eq:dr-lyap}. So any feasible $(P, K)$ for \eqref{eq:dr-stab-sdp}
    is feasible for \eqref{eq:stab-sdp}. The result then follows by \cref{prop:stablqr}. 
\end{proof}

We now consider the SDP relaxation of \cref{eq:dr-stab-sdp}:
\begin{proposition} \label{prop:dr-stab-sdp}
    Following the notation of \cref{cor:ambig}, 
    let $\covardr \dfn \covarh + \beta_\covar I$,  
    $F_i = A_i W_i + B_i V_i$ for $i \in \N_{1:\nwh}$, $\bm{F} \dfn [F_1; \dots; F_{n_w}]$, 
    $\hat{F} = \ssum_{i=1}^{n_w} [\meanh]_i F_i + F_{\nwh}$ and
    let $X_0 = U_0 \trans{U_0}$ denote the Cholesky factorization of $X_0$.

    Then consider the SDP:
    \begin{equation*}
        \begin{alignedat}{2}
            &\maximize_{W, V, S, \Lambda, \Gamma} &\quad& \tr[S] \\
            &\stt&& W \sgt 0, S \sgeq 0, \Lambda \sgeq 0, \Gamma \sgeq 0 \\
            &&& \begin{bmatrix}
                S & \trans{U_0} \\ U_0 & W
            \end{bmatrix} \sgeq 0, \, \begin{bmatrix}
                \Lambda & \beta_{\mean} \trans{\bm{F}} \\
                \beta_{\mean} \bm{F} & I_{n_w} \otimes \Gamma
            \end{bmatrix} \sgeq 0,\\
            &&& T \sgeq \blkdiag(\Lambda, 0, \Gamma, 0, 0),
        \end{alignedat}        
    \end{equation*}
    where we use the linear map:
    \begin{equation*}
        T \dfn \begin{bmatrix}
            W & \trans{\bm{F}} & \trans{\hat{F}} & W & \trans{V} \\
            \bm{F} & \covardr^{-1} \otimes W \\
            \hat{F} && W\\
            W &&& Q^{-1} \\
            V &&&& R^{-1}
        \end{bmatrix}.
    \end{equation*}
    Then given a feasible $(W, V)$, the pair $(P, K)$, with $P = W^{-1}$ and $K = VW^{-1}$, is feasible for
    \cref{eq:dr-stab-sdp}. As a result \cref{prop:stablqr-dr} is applicable for this pair. 
\end{proposition}
\begin{proof}
    We follow the proof of \cite[Thm.~10]{Coppens2019}. 
    % Writing out $\adj{\op{L}}(M, K; P)$ using \cref{lem:opadj} shows that \cref{eq:dr-lyap} holds iff:
    % \begin{align*}
    %     P &- (\ten{A}_{(2)} + \trans{K} \ten{B}_{(2)}) (M \otimes P) \trans{(\ten{A}_{(2)} + \trans{K} \ten{B}_{(2)})} \\
    %     &\sgeq \adj{\Pi}(K; H), \, \forall M \in \set{M}.
    % \end{align*}
    Note that $\nrm{\covar - \covarh}_2 \leq \beta_{\covar}$ iff $\covarh - \beta_{\covar} \sleq \covar \sleq \covardr$. 
    Since $M$ is linear in $\covar$ and $X \kron Y \sleq X' \kron Y$ if $X \sleq X'$, \eqref{eq:dr-lyap} holds iff:
    \begin{align}
        \adj{\op{L}}(\blkdiag(\covardr, 0) + \hm{\mean} \trans{\hm{\mean}}, K; P)  \sgeq \adj{\Pi}(K; H),\label{eq:dr-lyap-mean}
    \end{align}
    for all $\mean \in \set{C} \dfn \{ \mean \colon \nrm{\mean - \meanh}_2 \leq \beta_{\mean}\}$. By \cref{lem:opadj}, $\adj{\op{E}}(M; K)$ is:
    \begin{equation*}
        (\ten{A}_{(2)} + \trans{K} \ten{B}_{(2)}) (M \otimes P) \trans{(\ten{A}_{(2)} + \trans{K} \ten{B}_{(2)})}.
    \end{equation*}
    Hence, letting $W = P^{-1}$ and $V = KW$ and left-right multiplying \eqref{eq:dr-lyap-mean} with $W$ gives:
    \begin{align*}
        W &- \trans{[\bm{F}; F_{\nwh}]}(\hm{\mean} \otimes I) P (\trans{\hm{\mean}} \otimes I) [\bm{F}; F_{\nwh}] \\
        &- \trans{\bm{F}} (\covardr \otimes P) \bm{F}  \sgeq W Q W + \trans{V} R V,\, \forall \mean  \in \set{C}. 
    \end{align*}
    Applying a Schur complement, introducing $\theta \dfn \meanh - \mean$ and $T$ gives an inequality of the type $\op{U}[\beta_{\mean}] \sgeq 0$
    as in \cref{lem:rob-sdp}. Applying this, gives the second and third LMI in the final SDP. The cost still is $\tr[X_0 P] = \tr[\trans{U_0} P U_0]$
    which is rendered tractable using another Schur complement, producing the first LMI in the final SDP, thus completing the proof.
\end{proof}


Note that, by similarly introducing $W, V$ and applying suitable Schur complements, \eqref{eq:stab-sdp} can be 
reformulated as an SDP. Doing so illustrates that, for $\beta_{\mean} \to 0$ and $\beta_{\covar} \to 0$, the solution 
of the sdp in \cref{prop:dr-stab-sdp} converges to that of \eqref{eq:stab-sdp}. 
That is, \eqref{eq:dr-stab-sdp} somehow converges to \eqref{eq:stab-sdp} for larger $N$. 
